Fair Quantitative Games

We examine two-player games over finite weighted graphs with quantitative (mean-payoff or energy) objective, where one of the players additionally needs to satisfy a fairness objective. The specific fairness we consider is called 'strong transition fairness', given by a subset of edges of one of the players, which asks the player to take fair edges infinitely often if their source nodes are visited infinitely often. We show that when fairness is imposed on player 1, these games fall within the class of previously studied omega-regular mean-payoff and energy games. On the other hand, when the fairness is on player 2, to the best of our knowledge, these games have not been previously studied. We provide gadget-based algorithms for fair mean-payoff games where fairness is imposed on either player, and for fair energy games where the fairness is imposed on player 1. For all variants of fair mean-payoff and fair energy (under unknown initial credit) games, we give pseudo-polynomial algorithms to compute the winning regions of both players. Additionally, we analyze the strategy complexities required for these games. Our work is the first to extend the study of strong transition fairness, as well as gadget-based approaches, to the quantitative setting. We thereby demonstrate that the simplicity of strong transition fairness, as well as the applicability of gadget-based techniques, can be leveraged beyond the omega-regular domain.

==> sections/P1-fair-energy-old.tex <==
\begin{figure}
    \centering
     \includegraphics[width=0.6\linewidth]{figures/1-energy-gadget-drawing.jpg}
    \caption{Gadget}
  \end{figure}


  Here, we consider 1-fair energy games. 
  We once more use a gadget to 
  reduce the game into a regular energy game that have equivalent winning regions.

  \begin{theorem}
    Let $(G, E_f, \meanpayoff^f_0)$ be a 1-fair energy game where $G = (Q, E, w)$, $w : E \to [-W, W]$, and $|Q|=n$. Then there exists an energy game $G'= (Q',E',w')$ with $Q' \supseteq Q$, $|Q'|\leq 6n$. and $w' : E' \to [-W', W']$ with $W' = (n^2W+n)(n+1)$ such that
    $\Win_i(G) = \Win_i(G') \cap Q$ for $i \in \{1, 2\}$.
  \end{theorem}
  
   We call $G'$ the \emph{gadget game} and define it formally as $G' = (Q'_1, Q'_2, E', w')$ where
   \begin{align*}
    Q'_1 = &Q_1 \cup \{q_{-\varepsilon}, q_{\ESC}\, \mid \, q \in Q^f\}\\
    Q'_2 = &Q_2 \cup \{q_l, q_r, q_{nW+1}\, \mid \, q \in Q^f\}
   \end{align*}
   \begin{align*}
    E' \,= &\,\, \{\,qE  \,\mid\, q \not \in Q^f\,\}\, \cup \,\{\, (q, q_l),\, (q, q_r), \,(q_l, q_{nW+1}),\, (q_l, q_{-\varepsilon}),\, (q_r, q_{\ESC}) \,\mid \, q \in Q^f\,\} \\
    &\,\cup \,\{\, (q_{nW + 1}, p^f), \,(q_{-\varepsilon}, p),\, (q_{\ESC}, p) \, \mid \, q \in Q^f,\, p \in E(q) \text{ and } p^f \in E^f(q)\,\}
   \end{align*}
   and for $e = (q, p) \in E'$
   \begin{align*}
    W'(e) = \begin{cases}
    W(e) & q \not \in Q^f\\
     nW + 1 & p = u_{nW+1} \text{ for some } u \in Q, \\
     -\varepsilon & p = u_{-\varepsilon} \text{ for some } u \in Q, \\
     -n^2\cdot W -n & p = u_{\ESC} \text{ for some } u \in Q, \\
     W(u, p) &q\in \{u_{nW+1}, u_{-\varepsilon}, u_{\ESC}\} \text{ for some } u \in Q\\
     0 &\text{otherwise.}
    \end{cases}
   \end{align*}


  We call $G'$ the \emph{gadget game} and define it formally as $G' = (Q'_1, Q'_2, E', w')$ where
  \begin{align*}
   Q'_1 = &Q_1 \cup \{q_{0}, q_{\ESC}\, \mid \, q \in Q^f\}\\
   Q'_2 = &Q_2 \cup \{q_l, q_r, q_\text{nW+1}\, \mid \, q \in Q^f\}
  \end{align*}
  \begin{align*}
   E' \,= &\,\, \{\,qE  \,\mid\, q \not \in Q^f\,\}\, \cup \,\{\, (q, q_l),\, (q, q_r), \,(q_l, q_\text{nW+1}),\, (q_l, q_{0}),\, (q_r, q_{\ESC}) \,\mid \, q \in Q^f\,\} \\
   &\,\cup \,\{\, (q_\text{nW + 1}, p^f), \,(q_{0}, p),\, (q_{\ESC}, p) \, \mid \, q \in Q^f,\, p \in E(q) \text{ and } p^f \in E^f(q)\,\}
  \end{align*}
  and for $e = (q, p) \in E'$
  \begin{align*}
   w'(e) = \begin{cases}
   w(e) & q \not \in Q^f\\
    nW + 1 & p = u_\text{nW+1} \text{ for some } u \in Q, \\
    0 & p = u_{0} \text{ for some } u \in Q, \\
    -n^2\cdot W -n & p = u_{\ESC} \text{ for some } u \in Q, \\
    w(u, p) &q\in \{u_\text{nW+1}, u_{0}, u_{\ESC}\} \text{ for some } u \in Q\\
    0 &\text{otherwise.}
   \end{cases}
  \end{align*}


  For each $q \in Q^f$, we will denote the leftmost branch $q \to q_l \xrightarrow{nW+1} q_\text{nW+1}$ of the gadget with $\branch^q_{left}$, 
  the branch $q \to q_{l} \xrightarrow{0} q_{0}$ with $\branch^q_{0}$ and the rightmost branch 
  $q \to q_r \xrightarrow{-n^2\cdot W-n} q_{\ESC} $ with $\branch^q_{right}$. We will also call these branches \emph{left branch}, \emph{0 branch} and \emph{right branch}, respectively.
  
  We now prove the correctness of~\cref{thm:gadgetcorrectness}.
  \begin{proof}
    We first show $\Win_1(G') \, \cap \,Q \, \subseteq \,\Win_1(G)$, and then show $\Win_2(G') \, \cap \,Q \, \subseteq \,\Win_2(G)$.
    Due to determinacy of mean payoff games, as well as fair mean payoff games (defn. \ISin{complement winning condition}), 
    this gives us the winning regions of $G$.

    \smallskip
   $(\mathbf{\Win_1(G') \, \cap \,Q \, \subseteq \,\Win_1(G)}):$     Let $s'$ be a positional winning strategy of Player 1 in $G'$ that wins from $q$. 
   Consider the subgraph $G'_{s'}$ of $G'$. 
   Note that all cycles in $G'_{s'}$ are non-negative; because if a negative cycle exists in $G'_{s'}$, Player 2 
   has a strategy to force the game to eventually only see this cycle and therefore construct a play $\rho$ in $G'$ with negative mean payoff. This leads to a contradiction since $s'$ is winning for Player 1.

   Using $s'$, we construct a winning strategy $s$ for Player 1 in $G$ that wins from $q$ as follows:
   \begin{enumerate}[label=\alph*.]
       \item \label{item:zeroth} If $p \not \in Q^f$, then set $s$ to be positional at $p$ with $s(H \cdot p) = s'(p)$ for all histories $H \in Q^*$,
       \item \label{item:first} If $s'(p) = p_r$, then set $s$ to be positional at $p$ with $s(H \cdot p) = s'(p_{\ESC})$ for all histories $H \in Q^*$, 
       \item \label{item:second}
        Otherwise, with a local memory of size $\log(n^3W  +  n^2 + n+ |E^f(q)| + 1)$ make $s$ cycle through the set $\{s'(p_{0})\} \cup E^f(p)$ whenever it visits $p$, with a strategy that
       spends substantially longer time at $p$s \enquote{preferred successor} $s'(p_{0})$ to collect enough positive weight, before it cycles
       through its fair edges to fulfill the fairness condition. When $p$ is visited for the $k^{th}$ time, if $k \mod n^3W + n^2 + n + 1 \neq 0$, $s$ takes the edge $p \to s'(p_{0})$. 
       If $k \mod n^3W  + n^2 + n + 1 = 0$, $s$ takes an edge in $E^f(p)$, starting from an arbitrary fair edge and cycling through all of them one-by-one whenever this condition holds.
   \end{enumerate}

   We will show that any play $\rho$ that conforms with $s$ is winning for Player 1.
   
   \smallskip
   However, before we proceed we will introduce for a play $\rho = q^1 q^2 \ldots$ in $G$, \emph{the projection $\rho'$ of $\rho$ to $G'$}. The projection $\rho'$ is constructed inductively as follows: Starting from $ \rho' = q^1$ and $i = 1$, apply the corresponding rule listed below, increase $i$ by one, and repeat.
   \begin{itemize}
       \item If $q^i \not \in Q^f$, append $\rho'$ with $q^{i+1}$. Otherwise,
       \item If $s(H \cdot q^i)$ is defined using~\cref{item:first}, i.e. $s'(q^i) = q^i_r$; then append $\rho'$ with $\branch^{q^i}_{right} \to q^{i+1}$ i.e.
       append $\rho'$ with $q^i_r \cdot q^i_{\ESC}\cdot q^{i+1}$.
       \item If $s(H \cdot q^i)$ is defined using~\cref{item:second}, then if $q^{i+1} = s'(q^i_{0})$ append $\rho'$ with $\branch^{q^i}_{0} \to q^{i+1}$, i.e. $q^i_l \cdot q^i_{0} \cdot q^{i+1}$ ; 
       if not, append $\rho'$ with $\branch^{q^{i}}_{left} \to q^{i+1}$, i.e. $q^i_l \cdot q^i_\text{nW+1} \cdot q^{i+1}$. 
   \end{itemize}
   Clearly, $\rho'$ is a play in $G'_{s'}$. Furthermore, $\rho'$ restricted to \emph{non-gadget} nodes $Q'\setminus Q^{\gad} = Q$, is exactly $\rho$. We will 
   use the notation $\rho'|_Q = \rho$ to express this phenomenon.
   Next, we use the fact that $\rho'$ is a play in $G'_{s'}$, and therefore has only non-negative cycles,
   to show that $\rho$ is fair and $\MP(\rho) \geq 0$.

   Let's denote a tail of $\rho$ that consists only of the nodes and edges visited infinitely often in $\rho$ by $\sigma$; and the projection of $\sigma$ to $G'$ by $\sigma'$. We denote the subgame of $G'_{s'}$ restricted to the nodes and edges in $\sigma'$ by $G'_{\sigma'}$.
   We first show that $\rho$ is fair. To do so, it's sufficient to show that $\sigma$ (and therefore $\sigma'$)
   does not contain nodes for which $s$ is defined via~\cref{item:first}. This is because 
   every node in $\sigma$ for which $s$ is defined via~\cref{item:second} visits all their fair outgoing edges infinitely often in $\sigma$. 
   Let $p$ be a node for which $s$ is defined via~\cref{item:first}. Then $s'(p) = p_r$, i.e. from the branches of $p$, only $\branch^p_{right}$ exists in $G'_{\sigma'}$. This branch carries the weight $-n^2W - n$. 
   Since $p$ is visited infinitely often, there is a (simple) cycle in $G'_{\sigma'}$ that passes through $p$, and thus sees the weight $-n^2W -n$. This cycle must be non-negative
   since it's a cycle in $G'_{s'}$, but in order to be non-negative, it needs to visit $n$-many gadget edges with weight $nW+1$, which is not possible since there are at most $n-1$ many 
   gadget edges with this priority in $G'_{\sigma'}$. With this argument, we conclude that $\rho$ is fair.

   Before starting the proof of $\MP(\rho) \geq 0$ we make an observation about the cycles in $G'_{s'}$ that use only $0$ branches. 

   \smallskip
    \textit{Observation ($\varepsilon$-cycles).} Before we start the proof, we make an obervation about cycles in $G'_{s'}$ that use only $\varepsilon$-branches. As all cycles in $G'_{s'}$, these cycles have non-negative\ISin{positive} energy. 
    However, different from the other cycles, all the gadget nodes seen in such cycles have negative energy ($- \varepsilon$). Therefore, when we limit these cycles to non-gadget nodes $Q$, we get a non-negative, or positive energy\ISin{we get a positive energy} cycle in $G$.
    That is, if $\mathbf{c'}$ is a simple cycle in $G'$ s.t. all the gadget branches it contains are $\varepsilon$-branches, then $\mathbf{c}|_{Q}$ is a cycle in $G$ with $\energy(\mathbf{c}) \geq 0$\ISin{$\energy(\mathbf{c}) \geq 1$}. Moreover, if $\mathbf{c'}$ contains at least one $\varepsilon$-branch, then $\energy(\mathbf{c}) \geq 1$.

    \smallskip
   We have shown above that $\sigma'$ contains no nodes whose strategies are defined via~\cref{item:first}. Therefore, for all fair nodes $p$ in $\sigma$, $s$ is defined via~\cref{item:second}, and $G'_{\sigma'}$ contains only the branches $\branch^p_{left}$ and/or $\branch^p_{0}$.
   Thus, all cycles in $\sigma'$ are either $0$-cycles, or they visit a left branch. 

   If $\sigma$ contains no fair nodes, then $\sigma'$ and $\sigma$ are identical, and $\MP(\rho) \geq 0$ easily follows. Otherwise, since~\cref{item:second} is triggered infinitely often throughout $\sigma$, the value of counter $\mathbf{i}$ grows unboundedly. 
   
   To show $\MP(\sigma) \geq 0$ for such $\sigma$, we will use the following easy-to-verify fact: To prove $\MP(\omega) \geq \epsilon$ for an infinite play $\omega$ and a real number $\epsilon$, it is sufficient to prove 
   the existence a natural number $k$ and a tail $\omega_k$ of $\omega$ such that every $k$-length infix $\mathbf{v}$ of $\omega_k$ satisfies $\MP(\mathbf{v}) \geq \epsilon$.
   
   Since $\mathbf{i}$ grows unboundedly, for each round $i$, there exists a tail $\sigma_i$ of $\sigma$ such that 
   the value of $\mathbf{i}$ is $i$. In $\sigma_i$, the preferred successors (i.e., the $0$-branches) of fair nodes are visited at least $i$-many times in between two unpreferred successors (i.e., left branches).
   Therefore, in $\sigma_i$ each infix $\mathbf{v}$ of length $i$ visit the left branch of each node at most once. 
   Consequently, there are at most $n$-many simple cycles in $\mathbf{v}$ that visit a left branch, and all its other simple cycles are $0$-cycles.
   $n$-many non-$0$ simple cycles can produce the minimum weight of $-n^2W$, and since all the $0$-cycles have non-negative weight,
   $\MP(\mathbf{v}) \geq \frac{-n^2W}{i}$. Using the fact from the previous paragraph, we get that $\MP(\rho) = \MP(\sigma) \geq \frac{-n^2W}{i}$, and as 
   $\lim_{i\rightarrow \infty} \frac{-n^2W}{i} = 0$; we get $\MP(\rho) \geq 0$. \qed

   This concludes the proof of the first direction. Now let us prove the second direction. 


   \smallskip
   $(\mathbf{q \in \Win_2(G') \Rightarrow q \in \Win_2(G)}):$ As in the first direction, we take a positional Player 2 winning strategy $t'$ in $G'$ and construct, this time, a \emph{positional} Player 2 winning strategy $t$ in $G$.
   This time, the construction of $t$ is quite straight forward due to a lack of fair Player 2 nodes: For all $q \in Q_2$, we set $t(q) = t'(q)$. We define $G'_{t'}$ as before. 
   
   For a play $\rho = q^1 q^2 \ldots $ in $G$ that conforms with $t$, we define its projection $\rho'$ to $G'$. The projection function is quite different from the first direction.

   We construct $\rho'$ inductively as follows: Starting from $ \rho' = q^1$ and $i = 1$, apply the following step, increase $i$ by one, and repeat.
   \begin{itemize}
       \item If $q^i \not \in Q^f$, append $\rho'$ with $q^{i+1}$. Otherwise,
       \item If $\branch_{0}^{q^i}$ exists in $G'_{t'}$, append $\rho'$ with $q^i_l \cdot q^i_{0} \cdot q^{i+1}$,
       \item If $\branch_{0}^{q^i}$ does not exist in $G'_{t'}$:
       \begin{itemize} 
           \item If $q^{i+1} = t'(q^i_\text{nW+1})$, append $\rho'$ with the left branch i.e. $q^i_l \cdot q^i_\text{nW+1} \cdot q^{i+1}$, 
           \item Otherwise, append it with the right branch, i.e. $q^i_r \cdot q^i_{\ESC} \cdot q^{i+1}$.
       \end{itemize}
   \end{itemize}
   We define $\sigma$, $\sigma'$ and $G'_{\sigma'}$ as before. 

   Let $\rho$ be a play in $G$ that conforms with $t$. If $\rho$ is not fair, it is automatically won by Player 2. Therefore, assume that it is fair. We will use the fact that its projection $\rho'$ is a play in $G'_{t'}$, and therefore all the cycles in $G'_{\sigma'}$ have negative weight, 
   to show that all simple cycles in $\sigma$ have negative weight. Since the length of simple cycles are bounded by $n$, this automatically gives us $\MP(\rho) < 0$.

   Our main argument is the absence of left branches in $G'_{\sigma'}$, which we introduce in \emph{Claim 1}.
   The correctness of this argument implies all simple cycles in $\sigma$ having negative weight, and as we have seen, gives $\MP(\rho) < 0$.
   Before proving the claim, let's see why the claim leads to the mentioned outcome.
   By the definition of the projection, a lack of left branches implies that either (i) for all $q \in Q^f$ only $\branch^{q}_{0}$ exists in $G'_{\sigma'}$, or
    (ii) for some $q \in Q^f$, only the right branch $\branch^q_{right}$ exists in $\sigma'$. By construction of $\rho'$, (ii) implies that such $q$ appear infinitely often in $\rho$ but do not take all their fair outgoing edges, in particular $q \to t'(q_\text{nW+1}) \in E^f(q)$
    infinitely often. This implies that $\rho$ is unfair, contradicting our assumption. In case of (i), since all simple cycles $\mathbf{c}'$ in $\sigma'$ are negative and non of the gadget nodes contribute any weight due to only $0$-branches being seen, we conclude that the corresponding cycles $\mathbf{c} = \mathbf{c'}|_{Q}$ in $\sigma$
    have negative weight. By the above-mentioned argument, this gives us $\MP(\rho) < 0$.

    Now let's introduce and prove the claim. 
    
    \smallskip 
    \noindent \textit{Claim 1.} If $\rho$ is fair, there exist no $\branch_{left}$ in $G'_{\sigma'}$.

    \smallskip
   \noindent \textit{Proof of Claim 1.} As we have discussed above, since $\rho$ is fair, whenever $\branch^q_{right}$ is in $G'_{\sigma'}$ for a node $q \in Q^f$, $\branch^q_{left}$ is also in $G'_{\sigma'}$.
    Therefore, we can remove all the right branches $\branch^q_{right}$ of all nodes $q \in Q^f$ from $G'_{\sigma'}$ and receive a subgraph. Let's call this subgraph $S$. Note that $S$ has no dead-ends,
   since for all $q$ for which $\branch^q_{right}$ got removed, $\branch^q_{left}$ was also in $G'_{\sigma'}$, and therefore it is in $S$.
   For all nodes $q$ in $S$, either its left branch, or its $0$-branch is in $S$. Note that since it is a subgraph of $G'_{t'}$, all cycles in $S$ still have negative weight.
   It is easy to see that a node $q$ for which $\branch^q_{left}$ is in $S$ cannot lie on a cycle in $S$. That's because 
   this branch carries weight $nW+1$ and other edges in the cycle either are in $Q$, and therefore can have weight at least $-W$, or are gadget edges and have $0$-weight.
   Therefore any simple cycle such a branch lies on would have positive weight $\geq nW+1 - nW$.
   
   Now assume left branches exist in $\sigma'$, but not on cycles in $S$. Then all cycles in $S$ consist only of $0$-branches. However, nodes with $0$-branches
   have the same outgoing edges in 
   $G'_{\sigma'}$ as in $S$. Recall that every node in $S$ is visited infinitely often in $\rho$. Since $S$ has no dead-ends, it contains a cycle. 
   Then $\rho$ will eventually visit a node on a cycle of $S$. Since this node will have the same outgoing edges in $S$ and $\sigma'$, $\rho$ will never leave the cycles of $S$, which only have $0$-branches. 
   This implies that left branches are not visited after some point on in $\rho$, and contradicts our assumption that left branches exist in $\sigma'$.
   \qed
   With this, we conclude the proof of the second direction, and that of the theorem.
\end{proof}



  \begin{comment}
  \begin{theorem}\label{thm:gadgetcorrectness}
    Let $(G, E_f)$ be a fair energy game under unknown initial credit problem, with $G = (Q_1, Q_2, E, w)$ and $w : E \to [-W, W]$ where the number of nodes in $Q = Q_1 \cup Q_2$ is $n$. Then there exists an energy game $G'$ over the node set $Q' \supseteq Q$ over $\leq 6n$ nodes, edge set $E'$ and weight function $w' : E' \to [-W, W]\, \cup\, \{nW+1, -n^2W-n, -\varepsilon\}$ that satisfies for $i \in \{1, 2\}$ and every $q \in Q$, $q \in \Win_i(G)$ if and only if $q \in \Win_i(G')$.
  \end{theorem}
   We call $G'$ the \emph{gadget game} and define it formally as $G' = (Q'_1, Q'_2, E', w')$ where
   \begin{align*}
    Q'_1 = &Q_1 \cup \{q_{-\varepsilon}, q_{\ESC}\, \mid \, q \in Q^f\}\\
    Q'_2 = &Q_2 \cup \{q_l, q_r, q_{nW+1}\, \mid \, q \in Q^f\}
   \end{align*}
   \begin{align*}
    E' \,= &\,\, \{\,qE  \,\mid\, q \not \in Q^f\,\}\, \cup \,\{\, (q, q_l),\, (q, q_r), \,(q_l, q_{nW+1}),\, (q_l, q_{-\varepsilon}),\, (q_r, q_{\ESC}) \,\mid \, q \in Q^f\,\} \\
    &\,\cup \,\{\, (q_{nW + 1}, p^f), \,(q_{-\varepsilon}, p),\, (q_{\ESC}, p) \, \mid \, q \in Q^f,\, p \in E(q) \text{ and } p^f \in E^f(q)\,\}
   \end{align*}
   and for $e = (q, p) \in E'$
   \begin{align*}
    W'(e) = \begin{cases}
    W(e) & q \not \in Q^f\\
     nW + 1 & p = u_{nW+1} \text{ for some } u \in Q, \\
     -\varepsilon & p = u_{-\varepsilon} \text{ for some } u \in Q, \\
     -n^2\cdot W -n & p = u_{\ESC} \text{ for some } u \in Q, \\
     W(u, p) &q\in \{u_{nW+1}, u_{-\varepsilon}, u_{\ESC}\} \text{ for some } u \in Q\\
     0 &\text{otherwise.}
    \end{cases}
   \end{align*}

   This construction is depicted in~\cref{fig:gadget}. We will call $Q' \setminus Q$, \emph{gadget nodes}, and denote them with $Q^\gad$. We will
   similarly call the edges that exist due to the gadget, \emph{gadget edges}, denote them with $E^\gad := E' \setminus (\,E \,\cup \,\{\,(u_t, p) \, \mid \, u_t \in \{u_{nW+1}, u_{-\varepsilon}, u_{\ESC}\}\, \}\,)$.

   Each $q \in Q^f$ is replaced with the gadget in~\cref{fig:gadget}. For each $q \in Q^f$, we will denote the leftmost branch $q \to q_l \xrightarrow{nW+1} q_{nW+1}$ of the gadget with $\branch^q_{left}$, 
   the branch $q \to q_{l} \xrightarrow{-\varepsilon} q_{-\varepsilon}$ with $\branch^q_{-\varepsilon}$ and the rightmost branch 
   $q \to q_r \xrightarrow{-n^2\cdot W-n} q_{\ESC} $ with $\branch^q_{right}$. 
   
   We now prove the correctness of~\cref{thm:gadgetcorrectness}.
   \begin{proof}
    We will first prove the direction $\Rightarrow$, i.e. for all $q \in Q$, $q \in \Win_1(G') \Rightarrow q \in \Win_1(G)$. Then we will show the other direction via its contrapositive, i.e.
    for all $q \in Q$, $q \in \Win_2(G') \Rightarrow q \in \Win_2(G)$. By determinacy, this will give us the equivalence of winning regions of $G$ and $G'$, restricted to the node set $Q$.
   
    \smallskip
    $(\mathbf{q \in \Win_1(G') \Rightarrow q \in \Win_1(G)}):$ Let $s'$ be a positional winning strategy of Player 1 in $G'$ that wins from $q$. Denote the 
    game graph $G'$ where Player 1 nodes are restricted to their outgoing edges in $s'$ by $G'_{s'}$. 
    Note that all cycles in $G'_{s'}$ are non-negative; because if a negative cycle exists in $G'_{s'}$, Player 2 
    has a strategy to force the game to eventually only see this cycle and therefore construct a play in $G'$ that conforms with $s'$ with a total energy below zero after some point, for any initial credit. This is not possible since $s'$ is winning for Player 1.

    Using $s'$, we construct a winning strategy $s$ for Player 1 in $G$ that wins from $q$ as follows:
    \begin{enumerate}[label=\alph*.]
        \item \label{item:first} If $s'(p) = p_r$, then set $s$ to be positional at $p$ with $s(h \cdot p) = s'(p_{\ESC})$ for all histories $h \in Q^*$, 
        \item \label{item:second} Otherwise, with a local memory of size $\log(n^3W  +  n + |E^f(q)| + 2)$ make $s$ cycle through the set $\{s'(p_{-\varepsilon})\} \cup E^f(p)$ whenever it visits $p$, with a strategy that
        spends substantially longer time at $p$s \enquote{preferred successor} $s'(p_{-\varepsilon})$ to collect enough positive weight, before it cycles
        through its fair edges to fulfill the fairness condition. When $p$ is visited for the $k^{th}$ time, if $k \mod n^3W + n +2 \neq 0$, $s$ takes the edge $p \to s'(p_{-\varepsilon})$. 
        If $k \mod n^3W  + n +2 = 0$, $s$ takes an edge in $E^f(p)$, starting from an arbitrary fair edge and cycling through all of them one-by-one whenever this condition holds.
    \end{enumerate}

    We now show that there exists an initial credit $c$ such that for any play $\rho = q^1 q^2 \ldots $ in $G$ that conforms with $s$, $\rho$ is fair and $c + \energy(\rho_i) \geq 0$ for every prefix $\rho_i$ of $\rho$.
    
    Before we proceed we will introduce \emph{the projection $\rho'$ of $\rho$ to $G'$}. We construct $\rho'$ inductively as follows: Starting from $ \rho' = q^1$ and $i = 1$, apply the following step, increase $i$ by one, and repeat.
    \begin{itemize}
        \item if $q^i \not \in Q^f$, append $\rho'$ with $q_{i+1}$. Otherwise,
        \item if $s(h \cdot q^i)$ is defined using~\cref{item:first}, i.e. $s'(q^i) = q^i_r$; then append $\rho'$ with the right branch $\branch^{q^i}_{right} \to q^{i+1}$ i.e.
        append $\rho'$ with $q^i_r \cdot q^i_{\ESC}\cdot q^{i+1}$.
        \item if $s(h \cdot q^i)$ is defined using~\cref{item:second}, then if $q^{i+1} = s'(q^i_{-\varepsilon})$ append $\rho'$ with $\branch^{q^i}_{-\varepsilon} \to q^{i+1}$, i.e. $q^i_l \cdot q^i_{-\varepsilon} \cdot q^{i+1}$ ; 
        if not, append $\rho'$ with $\branch^{q^{i}}_{left} \to q^{i+1}$, i.e. $q^i_l \cdot q^i_{nW+1} \cdot q^{i+1}$. 
    \end{itemize}
    Clearly, $\rho'$ is a play in $G'_{s'}$. Furthermore, $\rho'$ restricted to \emph{non-gadget} nodes $Q'\setminus Q^{\gad} = Q$, is exactly $\rho$. We will 
    use the notation $\rho'|_Q = \rho$ to express this phenomenon.
    Next, we use the fact that $\rho'$ is a play in $G'_{s'}$, and therefore has only non-negative \ISin{positive} cycles,
    to show that $\rho$ is fair and there exists an initial credit $c$ with the desired property.

    Let's call a tail of $\rho$ that consists only of the cycles visited infinitely often in $\rho$, $\sigma$; and the projection of $\sigma$ to $G'$, $\sigma'$. We denote the subgame of $G'_{s'}$ restricted to the nodes and edges in $\sigma'$ by $G'_{\sigma'}$.
    We first show that $\rho$ is fair. To do so, it's sufficient to show that $\sigma$ (and therefore $\sigma'$)
    does not contain nodes for which $s$ is defined via~\cref{item:first}. This is because the way $s$ is defined in~\cref{item:second}
    guarantees the fairness on these nodes. 
    Let $p$ be a node for which $s$ is defined via~\cref{item:first}. Then $s'(p) = p_r$, i.e. from the branches of $p$, only $\branch^p_{right}$ exists in $G'_{\sigma'}$. This branch carries the weight $-n^2W - n$. 
    Since $p$ is visited infinitely often, there is a (simple) cycle in $G'_{\sigma'}$ that passes through $p$, and thus sees the weight $-n^2W -n$. This cycle must be non-negative \ISin{positive}
    since it's a cycle in $G'_{s'}$, but in order to be \ISin{even} non-negative with the weight in $w'$, it needs to visit $n$-many gadget edges with weight $nW+1$, which is not possible since there are at most $n-1$ many 
    gadget edges with this priority in $G'_{\sigma'}$. This concludes that $\rho$ is fair.

    Next, we need to show the existence of an initial credit $c$ s.t. $c + \energy(\rho_i) \geq 0 $ for all $\rho$ that conform with $s$ and $i \in \mathbb{N}$ \ISin{such that the limit of $\energy(\rho_i)$ is infinity.}. 
    Instead of this, we will show that $\energy(\sigma_i) \geq 0$ for all $i \in \mathbb{N}$. Which will imply the existence of such an initial credit. \ISin{Instead we will show it for the limit of $\energy(\sigma_i)$}\ISinside{This is not really enough as it is, to show the existence of an initial credit. We need to strenghten this argument, e.g. by limiting the size of $\rho-\sigma$ for all $\rho$ that conforms with $s$.}

    \smallskip
    \textit{Observation ($\varepsilon$-cycles).} Before we start the proof, we make an obervation about cycles in $G'_{s'}$ that use only $\varepsilon$-branches. As all cycles in $G'_{s'}$, these cycles have non-negative\ISin{positive} energy. 
    However, different from the other cycles, all the gadget nodes seen in such cycles have negative energy ($- \varepsilon$). Therefore, when we limit these cycles to non-gadget nodes $Q$, we get a non-negative, or positive energy\ISin{we get a positive energy} cycle in $G$.
    That is, if $\mathbf{c'}$ is a simple cycle in $G'$ s.t. all the gadget branches it contains are $\varepsilon$-branches, then $\mathbf{c}|_{Q}$ is a cycle in $G$ with $\energy(\mathbf{c}) \geq 0$\ISin{$\energy(\mathbf{c}) \geq 1$}. Moreover, if $\mathbf{c'}$ contains at least one $\varepsilon$-branch, then $\energy(\mathbf{c}) \geq 1$.

    \smallskip
    
    We have shown above that $\sigma'$ contains no nodes whose strategies are defined via~\cref{item:first}. Therefore, $G'_{\sigma'}$ contains only the branches $\branch_{left}$ and/or $\branch_{-\varepsilon}$ of all nodes  in $G'_{\sigma'}$.
    
    We will fix an arbitrary node $v \in \sigma$ and show that in between each $2$ occurence of $v$s leftmost branch $\branch^v_{left}$ in $\sigma'$, which corresponds to 
    every time the edge $v \to v'$ is taken in $\sigma$ where $v'$ is not the preferred successor of $v$, the total energy is non-negative\ISin{positive}. Furthermore, it will be clear from the argument that if for all nodes in $\sigma \cap Q^f$ their 
    non-preferred successors are seen only finitely often in $\sigma$, then the total energy is monotonically increasing.

    First let $\mathbf{u'} = \branch^v_{left} \to u^0 \to u^1 \to \ldots u^k \to v$ be an infix of $\sigma'$ that starts and ends at $v$; where the branch following $\mathbf{u'}$ in $\sigma'$ is again $\branch^{v}_{left}$, and
    for no $u \in \sigma$ does $\branch^{u}_{left}$ is seen in $\mathbf{u'}$ twice. 
    In words, $\mathbf{u'}$ is an infix of $\sigma'$ inbetween two occurrences of the leftmost branch of $v$, and no other nodes 
    take their leftmost branches twice in $\mathbf{u'}$.
    Let $\mathbf{u} = \mathbf{u'}|_{Q}$, the image in $\mathbf{u'}$ in $G$. Clearly, $\mathbf{u}$ also starts and ends with $v$. We will show that $\energy(\mathbf{u}) \geq 0$\ISin{$\energy(\mathbf{u}) \geq 1$}. 
    Observe that at most $n$-many leftmost branches are seen in $\mathbf{u'}$. The rest of the branches are $\varepsilon$-branches.
    Also since $v$s leftmost branch is seen as the first edge and the following edge of $\mathbf{u'}$, 
    the construction of $s$ implies that $v$ is seen $n^2W + n + 1$\ISin{$+1$} times in $\mathbf{u'}$ (and in $\mathbf{u}$). So $\mathbf{u'}$ (and $\mathbf{u}$)
    consists of $n^2W + n$\ISin{$+1$}-many cycles on $v$, whereas at most $n$ of these are non-$\varepsilon$ cycles. 
    The image of $n$-many non-$\varepsilon$ cycles in $\mathbf{u'}$ can consist of at most $n^2$ nodes in $\mathbf{u}$ and therefore, can induce the least energy of $-n^2W$.
    However since the rest of the cycles on $v$ are $\varepsilon$-cycles and each contain at least one $\varepsilon$-branch, $\branch^v_{-\varepsilon}$; by our previous observation each has energy $\geq 1$.
    Therefore, the total energy of $\mathbf{u}$ is non-negative\ISin{positive}. 

    Now define $\mathbf{u'}$ and $\mathbf{u}$ as above, but let $\mathbf{u'}$ contain left branches $\branch^u_{left}$ of nodes $u \neq v$ multiple times. That is, there can be at most $n-1$ that take their leftmost branches more than once in $\mathbf{u'}$.
    We will show by induction that $\mathbf{u'}$ has positive energy.
    \smallskip
    \textit{Claim.} If there are $\leq n-k$-many nodes whose left branches are taken more than once in $\mathbf{u'}$ for some $k \in [1, n]$, then $\energy(\mathbf{u'}) > (k-1) n^2 W$.
    
    \textit{Proof of claim.} For the base case, we take $k = n$, that is, no left branches repeat in $\mathbf{u'}$. This reduces to the case introduced in the previous paragraph, where we showed $\energy(\mathbf{u'}) > (n-1)n^2W$. 
    As the inductive hypothesis, we assume the statement holds for $i \in [k+1, n]$, i.e. if $\mathbf{u'}$ has $\leq n-i$ nodes repeating their leftmost branches for some $i \in [k+1, n]$, then $\energy(\mathbf{u'}) > (i-1) n^2 W$. 
    In the inductive step we show it for $k$, i.e. if $\mathbf{u'}$ has $\leq n-k$ nodes repeating their leftmost branches, $\energy(u') > (k-1) n^2 W$.
    In a $\mathbf{u'}$ with $(n-k)$-many nodes repeating their leftmost branches, we can find infices $\mathbf{w^1}, \ldots, \mathbf{w^t}$ of $\mathbf{u'}$ for some $t \leq n-k$ such that each $\mathbf{w^i}$ starts with a leftmost branch of a node $w$ and ends with the same node, and the branch following $\mathbf{w^i}$ is again $\branch^{w_i}_{left}$. 
    Furthermore, $w_i \neq w_j$ for all $i \neq j \in [1, t]$. We can repeat this operation exhaustively such that if we remove the infices $\mathbf{w^1}, \ldots, \mathbf{w^t}$ from $\mathbf{u'}$, in the remaining sequence $\mathbf{u^{-}}:=\mathbf{u'} - (\mathbf{w^1}, \ldots, \mathbf{w^t})$, there are no repeating left branches. 

    
    Note that the left branch of $w_i$ can be taken multiple times in $\mathbf{w^i}$.
    If there is no leftmost branch repeating in $\mathbf{u'}$, then we obtain the desired inequality from the base case. 
    Otherwise, we can always find at least such infix, $\mathbf{w^1}$.
    If in a $\mathbf{w^i}$, the left branch of $w_i$ repeats, then we can view $\mathbf{w^i}$ as a concetanation $\mathbf{w^i}_1\cdot \mathbf{w^i}_2 \cdots \mathbf{w^i}_p$ such that each $\mathbf{w^i}_j$ for $j \in [1, p]$ starts with $\branch^{w_i}_{left}$, ends with $w_i$, and $\branch^{w_i}_{left}$ is not repeated.
    If the left branch of $w_i$ does not repeat in $\mathbf{w^i}$, then simply, $\mathbf{w^i} = \mathbf{w^i}_1$.
    Note that in each $\mathbf{w^i}_j$, there are at most $(n-k-1)$-nodes repeating their leftmost branches. 
    Then, by the inductive hypothesis, $\energy(\mathbf{w^i}_j) > (k+1) n^2 W$, and therefore  $\energy(\mathbf{w^i}) > p \cdot (k+1) n^2 W \geq (k+1) n^2 W $ for every $\mathbf{w^i}$.

    Recall that in $\mathbf{u^{-}}$ there are no repeating left branches. That is, there are at most $n$-many left branches. By an argument similar to before, we know that there can be at most $n$-many simple non-$\varepsilon$ cycles, and they can cause 
    at the worst, $-n^2W$ negative energy. This is because $\epsilon$-cycles have positive energy.
    Since we assumed $\mathbf{u^{-}}$ has at least one infix $\mathbf{w^1}$ with energy larger than $(k+1) n^2 W$; we get that $\energy(\mathbf{u'}) > (k+1) n^2 W - n^2 W = k n^2 W$.
    This finishes the proof of the claim. \qed

    If there are no nodes in $\sigma$ that take their left branch in $\sigma'$, then all cycles in $\sigma'$ are $\varepsilon$-cycles, and therefore every cycle in $\sigma$ have non-negative\ISin{positive} energy. 

    As $\sigma'$ can be seen as an infinite concetanation of infices $\mathbf{u'}$ of bounded size (due to the finiteness of $G'$), we can conclude that $\energy(\sigma)\geq 0$\ISin{$\energy(\sigma_i)$ goes to infinity in the limit} in both cases, which finalizes the proof of $(\Rightarrow)$.\ISinside{Not quite. We need a bit more. Explained above.} Now we prove the second direction.

    \smallskip
    $(\mathbf{q \in \Win_2(G') \Rightarrow q \in \Win_2(G)}):$ As before, we take a positional Player 2 winning strategy $t'$ in $G'$ and construct a \emph{positional} Player 2 winning strategy $t$ in $G$.
    This time, the construction of $t$ is quite straight forward: For all $q \in V_2$, we set $t(q) = t'(q)$. We define $G'_{t'}$ as before. 
    
    Once more, for a play $\rho$ in $G$ that conforms with $t$, we define its projection $\rho'$ to $G'$. The projection function is different than the proof of the first direction.

    We construct $\rho'$ inductively as follows: Starting from $ \rho' = q^1$ and $i = 1$, apply the following step, increase $i$ by one, and repeat.
    \begin{itemize}
        \item if $q^i \not \in Q^f$, append $\rho'$ with $q_{i+1}$. Otherwise,
        \item if $\branch_{-\varepsilon}^{q^i}$ exists in $G'_{t'}$, append $\rho'$ with $q^i_l \cdot q^i_{-\varepsilon} \cdot q^{i+1}$,
        \item if $\branch_{-\varepsilon}^{q^i}$ does not exist in $G'_{t'}$:
        \begin{itemize} 
            \item if $q^{i+1} = t'(q^i_{nW+1})$, append $\rho'$ with the left branch i.e. $q^i_l \cdot q^i_{nW+1} \cdot q^{i+1}$, 
            \item otherwise, append it with the right branch, i.e. $q^i_r \cdot q^i_{\ESC} \cdot q^{i+1}$.
        \end{itemize}
    \end{itemize}
    We define $\sigma$, $\sigma'$ and $G'_{\sigma'}$ as before. 

    Now let $\rho$ be a play in $G$ that conforms with $t$. If $\rho$ is not fair, it is automatically won by Player 2. Assume that it is fair. We will use the fact that its projection $\rho'$ is a play in $G'_{t'}$, and therefore all the cycles in $G'_{\sigma'}$ have negative weight, 
    to show that all cycles in $\sigma$ have negative\ISin{non-positive} weight, and therefore,\ISin{$\energy(\rho_i)$ does not go to infinity in the limit} for all initial credits $c$, there exists a prefix $\rho_i$ s.t. $c + \energy(\rho_i) < 0$. That is, $t$ is winning for Player 2.

    To show this, we will first claim that there exist no $\branch_{left}$ in $G'_{\sigma'}$. By the definition of the projection, this gives us that either (i) for all $q \in Q^f$ only $\branch^{q}_{-\varepsilon}$ exists in $G'_{\sigma'}$, or
     (ii) for some $q \in Q^f$, only the rightmost branch $\branch^q_{right}$ exists in $\sigma'$. By construction of $\rho'$, (ii) implies that such $q$ appear infinitely often in $\rho$ but do not take all their fair outgoing edges, in particular $q \to t'(q_{nW+1}) \in E^f(q)$
     infinitely often. This implies that $\rho$ is unfair, contradicting our assumption. In case of (i), since all simple cycles $\mathbf{c}'$ in $\sigma'$ are negative and the weight that comes from the gadget nodes is $\geq -n\cdot \varepsilon$, we conclude that the corresponding cycles $\mathbf{c} = \mathbf{c'}|_{Q}$ in $\sigma$
     have non-positive weight. By our assumption that $G$ is free of zero-cycles, this gives us that all simple cycles in $\sigma$ are negative, and therefore $\rho$ is winning for Player 2. \ISin{We don't need the assumption of freeness from zero cycles anymore. We conclude that the corresponding cycles (i.e. all cycles) in $\sigma$ have non-positive weight, and therefore the limit of $\energy(\sigma_i)$ does not go to infinity. I.e. $\rho$ is won by Player 2.}
     
     Now let's prove the claim. 
     
     \smallskip 
     \noindent \textit{Claim. } If $\rho$ is fair, there exist no $\branch_{left}$ in $G'_{\sigma'}$.

     \smallskip
    \noindent \textit{Proof of Claim.} As we have discussed above, since $\rho$ is fair, whenever $\branch^q_{right}$ is in $G'_{\sigma'}$ for a node $q \in Q^f$, $\branch^q_{left}$ is also in $G'_{\sigma'}$.
     Therefore, we can remove all the right branches $\branch^q_{right}$ of all nodes $q \in Q^f$ from $G'_{\sigma'}$ and receive a subgraph. Let's call this subgraph $H$. Note that $H$ has no dead-ends,
    since for all $q$ for which $\branch^q_{right}$ got removed, $\branch^q_{left}$ was also in $G'_{\sigma'}$, and therefore it is in $H$.
    For all nodes $q$ in $H$, either its left branch, or its $\varepsilon$-branch is in $H$. Note that since it is a subgraph of $G'_{t'}$, all cycles in $H$ still have negative weight.
    It is easy to see that a node $q$ for which $\branch^q_{left}$ is in $H$ cannot lie on a cycle in $H$. That's because 
    this branch carries weight $nW+1$ and other edges in the cycle either are in $Q$, and therefore can have weight at least $-W$, or are gadget edges and have weight $-\varepsilon$.
    Therefore any simple cycle such a branch lies on would have weight $\geq nW+1 - nW - n\cdot \varepsilon > 0$.
    Now assume left branches exist in $H$ but not on cycles. Then all cycles in $H$ consist only of $\varepsilon$-branches. However, nodes with $\varepsilon$-branches 
    constitute strongly connected components and they
    have the same outgoing edges in 
    $G'_{\sigma'}$ as in $H$. This implies that after some point on $\rho'$ enters one of these strongly connected components and never see a node with a left branch again. This contradicts our assumption that left branches exist in $\sigma'$.

    \smallskip
    This concludes the proof of $(\Leftarrow)$ and therefore, of~\cref{thm:gadgetcorrectness}. \qed


\end{proof}
\end{comment}

==> sections/P2-fair-energy-old.tex <==
\ISin{First give the alternative definition of winning condition from the Player 2 pov. $\rho$ is won by Player 2 iff $\energy(\rho_i)$ goes to negative infinity in the limit, where $\rho_i$ is the prefix of $\rho$ of length $i$.
Remember that here, the live edges are defined on Player 2.}
\begin{theorem}\label{thm:gadgetcorrectness}
    Let $(G, E_f)$ be a fair energy game under unknown initial credit problem, with $G = (Q_1, Q_2, E, w)$ and $w : E \to [-W, W]$ where the number of nodes in $Q = Q_1 \cup Q_2$ is $n$. Then there exists an energy game $G'$ over the node set $Q' \supseteq Q$ over $\leq 6n$ nodes, edge set $E'$ and weight function $w' : E' \to [-W, W]\, \cup\, \{-nW-1, n^2W+n, \varepsilon\}$ that satisfies 
    $\Win_i(G) = \Win_i(G') \cap Q$ for $i \in \{1, 2\}$.
  \end{theorem}
   We call $G'$ the \emph{gadget game} and define it formally as $G' = (Q'_1, Q'_2, E', w')$ where
   \begin{align*}
    Q'_1 = &Q_1 \cup \{q_l, q_r, q_{-nW-1}\, \mid \, q \in Q^f\}\\
    Q'_2 = &Q_2 \cup \{q_{\varepsilon}, q_{\ESC}\, \mid \, q \in Q^f\}
   \end{align*}
   \begin{align*}
    E' \,= &\,\, \{\,qE  \,\mid\, q \not \in Q^f\,\}\, \cup \,\{\, (q, q_l),\, (q, q_r), \,(q_l, q_{-nW-1}),\, (q_l, q_{\varepsilon}),\, (q_r, q_{\ESC}) \,\mid \, q \in Q^f\,\} \\
    &\,\cup \,\{\, (q_{-nW-1}, p^f), \,(q_{\varepsilon}, p),\, (q_{\ESC}, p) \, \mid \, q \in Q^f,\, p \in E(q) \text{ and } p^f \in E^f(q)\,\}
   \end{align*}
   and for $e = (q, p) \in E'$
   \begin{align*}
    W'(e) = \begin{cases}
    W(e) & q \not \in Q^f\\
     -nW - 1 & p = u_{-nW-1} \text{ for some } u \in Q, \\
     \varepsilon & p = u_{\varepsilon} \text{ for some } u \in Q, \\
     n^2\cdot W +n & p = u_{\ESC} \text{ for some } u \in Q, \\
     W(u, p) &q\in \{u_{-nW-1}, u_{\varepsilon}, u_{\ESC}\} \text{ for some } u \in Q\\
     0 &\text{otherwise.}
    \end{cases}
   \end{align*}

   \begin{figure}
    \centering
     \includegraphics[width=0.6\linewidth]{figures/Player2-gadget.jpg}
    \caption{Gadget}
    \label{fig:gadget}
  \end{figure}

   This construction is depicted in~\cref{fig:gadget}. We will call $Q' \setminus Q$, \emph{gadget nodes}, and denote them with $Q^\gad$. We will
   similarly call the edges that exist due to the gadget, \emph{gadget edges}, denote them with $E^\gad := E' \setminus (\,E \,\cup \,\{\,(u_t, p) \, \mid \, u_t \in \{u_{-nW-1}, u_{\varepsilon}, u_{\ESC}\}\, \}\,)$.%\ISinside{I am not sure if we use "gadget edges" anywhere}

   Each $q \in Q^f$ is replaced with the gadget in~\cref{fig:gadget}. That is, the incoming edges of $q$ are directed to node $q$ on top of the gadget,
   nodes $q_{\varepsilon}$ and $q_{\ESC}$ has as successors, the successors of q; and $q_{-nW-1}$ has as successors the fair successors of $q$.
   For each $q \in Q^f$, we will denote the leftmost branch $q \to q_l \xrightarrow{-nW-1} q_{-nW-1}$ of the gadget with $\branch^q_{left}$, 
   the branch $q \to q_{l} \xrightarrow{\varepsilon} q_{\varepsilon}$ with $\branch^q_{\varepsilon}$ and the rightmost branch 
   $q \to q_r \xrightarrow{n^2\cdot W+n} q_{\ESC} $ with $\branch^q_{right}$. 
   
   We now prove the correctness of~\cref{thm:gadgetcorrectness}.
   \begin{proof}
    Due to the determinacy of energy games, showing $\Win_1(G)\, = \,\Win_1(G') \,\cap\, Q$ is sufficient to prove the equivalence of the winning regions in $G$ and $G'$, restricted to $Q$. 
    We will first prove the direction $\supseteq$, i.e. for all $\Win_1(G') \, \cap \, Q\,\subseteq\, \Win_1(G)$. Then we will show the other direction via its contrapositive, i.e.
    for all $\Win_2(G')\, \cap\, Q \,\subseteq \,\Win_2(G)$.
    
    \smallskip
    $(\mathbf{\Win_1(G') \, \cap \,Q \, \subseteq \,\Win_1(G)}):$ Recall that both players have positional strategies in energy games\ISinside{define positional strategies.}.
    Let $s'$ be a positional winning strategy of Player 1 in $G'$. Denote the 
    game graph $G'$ where Player 1 nodes are restricted to their outgoing edges in $s'$ by $G'_{s'}$. 
    Note that since Player 1 has a unique outgoing edge from each of its nodes, $G'_{s'}$ is a one-player game for Player 2.
    This implies that all cycles in $G'_{s'}$ are non-negative; because if a negative cycle exists in $G'_{s'}$, Player 2 
    can force the game to eventually only take this cycle. This would give a Player 2 strategy that wins a play compliant with $s'$, which is a contradiction. 

    Using $s'$, we will construct a \emph{positional} Player 1 winning strategy $s$ in $G$.
    The construction of $s$ is quite straight forward: For all $q \in V_1$, we set $s(q) = s'(q)$.

    We introduce \emph{the projection $\rho'$ of $\rho = q_1 q_2 \ldots$ to $G'$}.\ISinside{should i add that $\rho$ is compliant with $s$} We construct $\rho'$ inductively as follows: Starting from $ \rho' = q^1$ and $i = 1$, apply the following step, increase $i$ by one, and repeat.
    %For a play $\rho$ in $G$ that conforms with $s$, we define its projection $\rho'$ to $G'$ inductively as follows:
    %Starting from $ \rho' = q^1$ and $i = 1$, apply the following step, increase $i$ by one, and repeat.
    \begin{itemize}
        \item if $q^i \not \in Q^f$, append $\rho'$ with $q_{i+1}$. Otherwise,
        \item if $\branch_{\varepsilon}^{q^i}$ exists in $G'_{s'}$, append $\rho'$ with $q^i_l \cdot q^i_{-\varepsilon} \cdot q^{i+1}$,
        \item if $\branch_{\varepsilon}^{q^i}$ does not exist in $G'_{s'}$:
        \begin{itemize} 
            \item if $q^{i+1} = s'(q^i_{-nW-1})$, append $\rho'$ with the left branch i.e. $q^i_l \cdot q^i_{-nW-1} \cdot q^{i+1}$, 
            \item otherwise, append it with the right branch, i.e. $q^i_r \cdot q^i_{\ESC} \cdot q^{i+1}$.
        \end{itemize}
    \end{itemize}

    Clearly, $\rho'$ is a play in $G'_{s'}$. Furthermore, $\rho'$ restricted to \emph{non-gadget} nodes $Q'\setminus Q^{\gad} = Q$, is exactly $\rho$. We will 
    use the notation $\rho'|_Q = \rho$ to express this phenomenon.
    Next, we use the fact that $\rho'$ is a play in $G'_{s'}$, and therefore has only non-negative cycles,
    to show that either (i) $\rho$ is unfair, or (ii) $\liminf_{i \to \infty} \energy(\rho_i) \not \to -\infty$.

    We call a tail of $\rho$ that consists only of the cycles visited infinitely often in $\rho$, $\sigma$; and the projection of $\sigma$ to $G'$, $\sigma'$. We denote the subgame of $G'_{s'}$ restricted to the nodes and edges in $\sigma'$ by $G'_{\sigma'}$.
    
    Now let $\rho$ be a play in $G$ that conforms with $s$. If $\rho$ is not fair, we are in case (i) and $\rho$ is won by Player 1. Therefore we assume that $\rho$ is fair. We will use the fact that its projection $\rho'$ is a play in $G'_{s'}$, and therefore all the cycles in $G'_{\sigma'}$ have non-negative weight, 
    to show that all cycles in $\sigma$ have non-negative weight, and therefore
    $\liminf_{i \to \infty} \energy(\rho_i) \not \to -\infty$. \ISinside{This is because the length of simple cycles is bounded. Should I explain more?} 

    To show this, we will first claim that there exist no $\branch_{left}$ in $G'_{\sigma'}$. By the definition of the projection, this gives us that either (i) for all $q \in Q^f$ only $\branch^{q}_{\varepsilon}$ exists in $G'_{\sigma'}$, or
     (ii) for some $q \in Q^f$, only the rightmost branch $\branch^q_{right}$ exists in $\sigma'$. By construction of $\rho'$, (ii) implies that such $q$ appear infinitely often in $\rho$ but do not take all their fair outgoing edges, in particular $q \to s'(q_{-nW-1}) \in E^f(q)$
     infinitely often. This implies that $\rho$ is unfair, contradicting our assumption. In case of (i), since all simple cycles $\mathbf{c}'$ in $\sigma'$ are non-negative and the weight that comes from the gadget nodes is $\leq n\cdot \varepsilon < 1$, we conclude that the corresponding cycles $\mathbf{c} = \mathbf{c'}|_{Q}$ in $\sigma$
     have non-negative weight. Since after some point on, all simple cycles in $\rho$ have non-negative weight, $\energy(\rho_i)$ does not go to $- \infty$ in the limit. Therefore, 
      $\rho$ is winning for Player 1. 

     Now let's prove the claim. 
     
     \smallskip 
     \noindent \textit{Claim. } If $\rho$ is fair, there exist no $\branch_{left}$ in $G'_{\sigma'}$.

     \smallskip
    \noindent \textit{Proof of Claim.} As we have discussed above, since $\rho$ is fair, whenever $\branch^q_{right}$ is in $G'_{\sigma'}$ for a node $q \in Q^f$, $\branch^q_{left}$ is also in $G'_{\sigma'}$.
     Therefore, we can remove all the right branches $\branch^q_{right}$ of all nodes $q \in Q^f$ from $G'_{\sigma'}$ and receive a subgraph. Let's call this subgraph $H$. Note that $H$ has no dead-ends,
    since for all $q$ for which $\branch^q_{right}$ got removed, $\branch^q_{left}$ was also in $G'_{\sigma'}$, and therefore it is in $H$.
    For all nodes $q$ in $H$, either its left branch, or its $\varepsilon$-branch is in $H$. Recall that since it is a subgraph of $G'_{s'}$, all cycles in $H$ have non-negative weight.
    It is easy to see that a node $q$ for which $\branch^q_{left}$ is in $H$ cannot lie on a cycle in $H$. That's because 
    this branch carries the weight $-nW-1$ and other edges in the cycle either are in $Q$, and therefore can have weight at most $W$, or are gadget edges and have weight $\varepsilon$.
    Therefore any simple cycle such a branch lies on would have weight $\leq  nW + n\cdot \varepsilon - nw - 1 < 0$.
    Now assume left branches exist in $\sigma'$, but not on cycles in $H$. Then all cycles in $H$ consist only of $\varepsilon$-branches. However, nodes with $\varepsilon$-branches
    have the same outgoing edges in 
    $G'_{\sigma'}$ as in $H$. Recall that every node in $H$ is visited infinitely often in $\rho$. Since $H$ has no dead-ends, it contains a cycle. 
    Then $\rho$ will eventually visit a node on a cycle of $H$. Since this node will have the same outgoing edges in $H$ and $\sigma'$, $\rho$ will never leave the cycles of $H$, which only have $\varepsilon$-branches. 
    This implies that left branches are not visited after some point in $\rho$, and contradicts our assumption that left branches exist in $\sigma'$.

    \smallskip
    This concludes the proof of the first direction. Now let's prove the second direction.

    \smallskip
    $(\mathbf{\Win_2(G') \, \cap \,Q  \subseteq \, \Win_2(G)}):$  Let $t'$ be a positional winning strategy of Player 2 in $G'$ and $G'_{t'}$ be the game graph restricted to strategy $t'$.  
    This time all cycles in $G'_{t'}$ have negative energy. As before, using $t'$, we will construct a winning Player 2 strategy $t$ in $G$. However, due to the live edges on Player 2 nodes, $t$ cannot be a positional strategy anymore. %Therefore, the construction will be more complicated.
    \begin{enumerate}[label=\alph*.]
        \item \label{item:first} If $t'(p) = p_r$, then set $t$ to be positional at $p$ with $t(h \cdot p) = s'(p_{\ESC})$ for all histories $h \in Q^*$, 
        \item \label{item:second} Otherwise, with a local memory of size $\log(n^3W  +  n + |E^f(q)| + 2)$ make $t$ cycle through the set $\{t'(p_{\varepsilon})\} \cup E^f(p)$ whenever it visits $p$, with a strategy that
        spends substantially longer time at $p$s \enquote{preferred successor} $t'(p_{\varepsilon})$ to collect enough positive weight, before it cycles
        through its fair edges to fulfill the fairness condition. When $p$ is visited for the $k^{th}$ time, if $k \mod n^3W + n +2 \neq 0$, $t$ takes the edge $p \to t'(p_{\varepsilon})$. 
        If $k \mod n^3W  + n +2 = 0$, $t$ takes an edge in $E^f(p)$, starting from an arbitrary fair edge and cycling through all of them one-by-one whenever this condition holds.
    \end{enumerate}

    %We now show that for a play $\rho$ compliant with $t$ in $G$, $\energy(\rho_i)$ goes to $-\infty$ in the limit. 

    Similar to the first direction, we define the projection $\rho'$ of a play $\rho = q^1 q^2 \ldots$ to $G'$.
    The projection function is different than the one in the first direction and we require the projected play $\rho$ to be compliant with $t$ for the projection to be well-defined. 
    We construct $\rho'$ inductively as follows: Starting from $\rho' = q^1$ and $i = 1$, apply the following step, increase $i$ by one, and repeat.
    \begin{itemize}
        \item if $q^i \not \in Q^f$, append $\rho'$ with $q_{i+1}$. Otherwise,
        \item if $t(h \cdot q^i)$ is defined using~\cref{item:first}, i.e. $t'(q^i) = q^i_r$; then append $\rho'$ with the right branch $\branch^{q^i}_{right} \to q^{i+1}$ i.e.
        append $\rho'$ with $q^i_r \cdot q^i_{\ESC}\cdot q^{i+1}$.
        \item if $t(h \cdot q^i)$ is defined using~\cref{item:second}, then if $q^{i+1} = t'(q^i_{\varepsilon})$ append $\rho'$ with $\branch^{q^i}_{\varepsilon} \to q^{i+1}$, i.e. $q^i_l \cdot q^i_{\varepsilon} \cdot q^{i+1}$ ; 
        if not, append $\rho'$ with $\branch^{q^{i}}_{left} \to q^{i+1}$, i.e. $q^i_l \cdot q^i_{-nW-1} \cdot q^{i+1}$. 
    \end{itemize}
    We inherit the definition of $\sigma$, $\sigma'$ and $G'_{\sigma'}$ from the proof of the first direction. 

    Once more, $\rho'|_Q = \rho$ and $\rho'$ is a play in $G'_{t'}$, therefore only has negative cycles. We will use this fact to show that (i) $\rho$ is fair, and (ii) $\liminf_{i \to \infty} \energy(\rho_i) \to -\infty$.

    We first show that (i) $\rho$ is fair. To do so, it's sufficient to show that $\sigma$ (and therefore $\sigma'$)
    does not contain nodes for which $t$ is defined via~\cref{item:first}. This is because the way $t$ is defined in~\cref{item:second}
    guarantees the fairness on these nodes. 
    Let $p$ be a node for which $t$ is defined via~\cref{item:first}. Then $t'(p) = p_r$, i.e. from the branches of $p$, only $\branch^p_{right}$ exists in $G'_{\sigma'}$. This branch carries the weight $n^2W + n$. 
    Since $p$ is visited infinitely often, there is a (simple) cycle in $G'_{\sigma'}$ that passes through $p$, and thus sees the weight $n^2W +n$. This cycle must be negative
    since it's a cycle in $G'_{t'}$, but in order to be non-positive, it needs to visit $n$-many gadget edges with weight $-nW-1$, which is not possible since due to $p$ taking its right branch in $G_{\sigma'}$, there are at most $n-1$  
    gadget edges with weight $-nW-1$ in $G'_{\sigma'}$. This concludes that $\rho$ is fair.


    Before starting the proof of (ii) $\liminf_{i \to \infty} \energy(\rho_i) \to -\infty$ we make an observation about the cycles in $G'_{t'}$ that use only $\varepsilon$-branches. 

    \smallskip
    \textit{Observation ($\varepsilon$-cycles).} As all cycles in $G'_{t'}$, these cycles have negative energy. 
    However, differently from the other cycles, all the gadget nodes seen in such cycles have the positive weight $\varepsilon$. Therefore, when we limit these cycles to non-gadget nodes $Q$, we get negative energy cycles in $G$.
    That is, if $\mathbf{c'}$ is a simple cycle in $G'$ s.t. all the gadget branches it contains are $\varepsilon$-branches, then $\mathbf{c} = \mathbf{c'}|_{Q}$ is a cycle in $G$ with $\energy(\mathbf{c}) \leq -1$.

    We have shown above that $\sigma'$ contains no nodes whose strategies are defined via~\cref{item:first}. Therefore, $G'_{\sigma'}$ contains only the branches $\branch_{left}$ and/or $\branch_{\varepsilon}$ of all nodes  in $G'_{\sigma'}$.
    
    We fix an arbitrary node $v \in \sigma$ such that $v$s leftmost branch is in $\sigma'$; and show that in between each $2$ consecutive occurence of $\branch^v_{left}$ in $\sigma'$, which corresponds to 
    every time the edge $v \to v'$ is taken in $\sigma$ where $v'$ is not the preferred successor of $v$, the total energy is negative. Since for any such $v$, $\sigma$ can be viewed as a concetanation of simple cycles over the edge $v \to v'$. 
    By proving all such cycles have negative energy, we will have shown that $\liminf_{i \to \infty} \energy(\rho_i) = - \infty$, i.e. $\rho$ is winning for Player 2.
    This argument assumes that $\sigma'$ contains the left branch of at least one node. After we prove the claim, we will explain the easier case of $\sigma'$ being free of left branches. 
    
    \textit{Claim 1.}  Let $\mathbf{v'}$ be an infix of $\sigma'$ which starts and ends with a node $v$, starting with the left branch of $v$, the branch following $\mathbf{v'}$ in $\sigma'$ is again $\branch^v_{left}$ and $\branch^v_{left}$ is seen only once in $\mathbf{v'}$, that is, in the beginning.
    Then $\energy(\mathbf{v}) < 0$ for $\mathbf{v} = \mathbf{v'}|_G$.
    
    \textit{Proof of Claim 1.} 
    Even though $\branch^v_{left}$ does not repeat in $\mathbf{v'}$, other nodes' left branches might be seen arbitrarily many times in $\mathbf{v'}$. At most, there are $n-1$ nodes whose left branches are seen more than once in $\mathbf{v'}$. We will proceed by induction on 
    the number of such nodes. 
    We will show the following: If there are $\leq (n-k)$-many nodes whose left branches are taken more than once in $\mathbf{v'}$ for some $k \in [1, n]$, then $\energy(\mathbf{v'}) < - (k-1) n^2 W$.
    
    \textbf{Base case (k = n):} In this case, the left branches of all nodes are seen at most once in $\mathbf{v'}$.  
    That is, there are at most $n$-many leftmost branches seen in $\mathbf{u'}$ and the rest of the branches are $\varepsilon$-branches.
    Also since $v$s leftmost branch is seen as the first edge and the following edge of $\mathbf{v'}$, 
    the construction of $t$ implies that $v$ is seen $n^3W + n + 2$ times in $\mathbf{v'}$ (and in $\mathbf{v}$). So $\mathbf{v'}$ (and $\mathbf{v}$)
    consists of $n^3W + n + 1$-many cycles on $v$, whereas at most $n$ of these contain simple non-$\varepsilon$ cycles. 
    The image of $n$-many simple non-$\varepsilon$ cycles in $\mathbf{v'}$ can consist of at most $n^2$ nodes in $\mathbf{v}$ and therefore, can induce the maximum energy of $n^2W$.
    However since the rest of the cycles on $v$ are $\varepsilon$-cycles; by our previous observation each has energy $\leq -1$.
    Therefore, $\energy(\mathbf{v}) \leq - n^3W -1 + n^2W < - (n-1)n^2W$.

    \smallskip
    \textbf{Inductive Hypothesis:} Assume the statement holds for $i \in [k+1, n]$, i.e. if $\mathbf{v'}$ has $\leq n-i$ nodes repeating their leftmost branches for some $i \in [k+1, n]$, then $\energy(\mathbf{v'}) < - (i-1) n^2 W$. 

    \smallskip 
    \textbf{Inductive Step:} We will show that the statement holds for $i = k \neq n$. 
    We assume $\mathbf{v'}$ has exactly $(n-k)$ repeating leftmost branches, since if it has less than that we get the desired inequality from the inductive hypothesis.
    In such a $\mathbf{v'}$ we can find infices $\mathbf{w^1}, \ldots, \mathbf{w^t}$ for some $t \in [1, n-k]$ such that each $\mathbf{w^i}$ starts with a leftmost branch of a node $w$ and ends with the same node, and the branch following $\mathbf{w^i}$ is again $\branch^{w_i}_{left}$. 
    Furthermore, $w_i \neq w_j$ for all $i \neq j \in [1, t]$. We can repeat this operation exhaustively such that if we remove the infices $\mathbf{w^1}, \ldots, \mathbf{w^t}$ from $\mathbf{u'}$, in the remaining sequence $\mathbf{v^{-}}:=\mathbf{v'} - (\mathbf{w^1}, \ldots, \mathbf{w^t})$\ISinside{need to set up this (or some better) notation for this}, there are no repeating left branches. 

    Note that the left branch of $w_i$ can be taken multiple times in $\mathbf{w^i}$.
    If in a $\mathbf{w^i}$, the left branch of $w_i$ repeats, then we can view $\mathbf{w^i}$ as a concetanation $\mathbf{w^i}_1\cdot \mathbf{w^i}_2 \cdots \mathbf{w^i}_p$ such that each $\mathbf{w^i}_j$ for $j \in [1, p]$ starts with $\branch^{w_i}_{left}$, ends with $w_i$, and $\branch^{w_i}_{left}$ is not repeated.
    If the left branch of $w_i$ does not repeat in $\mathbf{w^i}$, then simply, $p = 1$.
    Observe that in each $\mathbf{w^i}_j$, there are at most $(n-(k+1))$-nodes repeating their leftmost branches. 
    Then, by the inductive hypothesis, $\energy(\mathbf{w^i}_j) < -k n^2 W$, and therefore  $\energy(\mathbf{w^i}) < - p \cdot k n^2 W \leq - k n^2 W $ for every $\mathbf{w^i}$.

    Recall that in $\mathbf{v^{-}}$ there are no repeating left branches. That is, there are at most $n$-many left branches in $\mathbf{v^{-}}$. Similar to the base case, we know that there can be at most $n$-many simple non-$\varepsilon$ cycles in $\mathbf{v^{-}}$, and they can  
    casue the maximum energy of $n^2W$. %This is because the rest of the cycles in $\mathbf{v^{-}}$ are $\varepsilon$-cycles and have negative energy.
    Since $\mathbf{v'}$ has at least one infix $\mathbf{w^1}$ with energy $ < - k n^2 W$; we get that $\energy(\mathbf{v'}) < - k n^2 W + n^2 W = - (k-1) n^2 W$.
    This finishes the induction, as well as the proof of the claim. \qed

    Finally we look into the case where $\sigma'$ does not contain any left branches. Then all cycles in $\sigma'$ are $\varepsilon$-cycles, and therefore every cycle in $\sigma$ has negative energy. 
    Once again we get that $\liminf_{i \to \infty} \energy(\rho_i) = - \infty$. This concludes the proof of the second direction, and therefore of~\cref{thm:gadgetcorrectness}. 

    

   \end{proof}

==> sections/algo.tex <==
Dummy citation to prevent error: \cite{knuth1984texbook}

In this section, we provide an algorithm to solve fair energy games.

\begin{itemize}
    \item By reduction to normal energy games, using Irmak's gadget!
    \item Prove that the gadget works
    \item Some intuition on how the combination of memoryless strategies works for Player $1$ in the original game without reduction to normal energy games
    \item Fixed point characterization
\end{itemize}

We first give a reduction from fair energy games to \enquote{normal} energy games, with the use of \emph{gadgets}, by inducing only a linear blowup in the state space and a polynomial increase in the maximum weight. 



==> sections/discussion-energy-determinacy.tex <==
\subsection{Determinacy of Fair Energy Games}\label{subsec:determinacyoffairenergy}
  
Recall that the winning regions in fair energy games are defined via~\Cref{eq:energyDeterminacyPlayer1,eq:energyDeterminacyPlayer2} where $\varphi_c = \energy^f_c$. As we will see in~\Cref{sec:2-fair-energy}, $\omega$-regular energy games are not determined in general. Therefore, authors have used the definition of player~2 winning region in~\Cref{eq:energyDeterminacyPlayer2-traditional} that ensures determinacy.  
\begin{equation}
  q \in \Win_2 \iff \forall c \in \mathbb{N}.  \exists \sigma \in \Sigma_2. \forall \pi \in \Sigma_1,  \play_{\sigma, \pi}(G, q) \not \in \varphi_c\label{eq:energyDeterminacyPlayer2-traditional}
\end{equation}

\Cref{eq:energyDeterminacyPlayer2-traditional} trivially ensures determinacy because it is equivalent to~\Cref{eq:energyDeterminacyPlayer2-trivial}, where $\Win_2$ is defined as the complement of~\Cref{eq:energyDeterminacyPlayer1}. The equivalence comes from Borel determinacy[] due to $\energy_c(G)$ being a Borel set. This allows us to swap the quantifiers over $\Sigma_1$ and $\Sigma_2$ strategies for a fixed $c$. 

\begin{equation}
  q \in \Win_2 \iff \forall c \in \mathbb{N}. \forall \pi \in \Sigma_1.  \exists \sigma \in \Sigma_2, \play_{\sigma, \pi}(G, q) \not \in \varphi_c\label{eq:energyDeterminacyPlayer2-trivial}
\end{equation}


Note that the equivalence of \Cref{eq:energyDeterminacyPlayer2-1} and \Cref{eq:energyDeterminacyPlayer2-2} is specific to energy games, and is not merely a logical equivalence. 

We immediately get the following equivalent formulation of \Cref{eq:energyDeterminacyPlayer2-1} from Borel determinacy due to $\energy_c(G)$ being a Borel set. The determinacy of the winning condition for a fixed $c$ allows us to swap the quantifiers over player~1 and player~2. 
\begin{equation}
  q \in \Win_2 \iff \forall c \in \mathbb{N}.  \exists \sigma \in \Sigma_2. \forall \pi \in \Sigma_1,  \play_{\sigma, \pi}(G, q) \not \in \varphi_c \label{eq:energyDeterminacyPlayer2-1-equivalent}
\end{equation}
Again due to Borel determinacy we get the equivalence of \Cref{eq:energyDeterminacyPlayer2-1} and \Cref{eq:energyDeterminacyPlayer2-2} if we can restrict $c$ to a finite set \ISin{more reasoning?}. This is reason why this equivalence holds for energy games: because in energy games, if there exists a player~2 strategy $\sigma$ that wins against all player~1 strategies for the initial credit $c = nW$, then $\sigma$ wins against all player~1 strategies for all initial credits. The positional determinacy of energy games (for both players), is an easy way to observe this fact.

However, in $\omega$-regular energy games the equivalence of \Cref{eq:energyDeterminacyPlayer2-1} and \Cref{eq:energyDeterminacyPlayer2-2} does not hold anymore, where $\varphi_c = \energy_c(G) \cap \Psi$ for an $\omega$-regular set $\Psi$. For an example consider the 2-fair energy game in~\Cref{fig:2-fair-energy-game}. Player 1 has no winning strategy from $q$ since there exists no initial credit it can enforce on a play that satisfies $\Psi$. Therefore, with respect to \Cref{eq:energyDeterminacyPlayer2-1}, $q$ is won by player~2. However, player~2 has no strategy that can win against all initial credits. Therefore, $q$ is not won by player~2 wrt \Cref{eq:energyDeterminacyPlayer2-2}. In existing work on $\omega$-regular energy games, researchers has adapted \Cref{eq:energyDeterminacyPlayer2-1} (or equivalently,\Cref{eq:energyDeterminacyPlayer2-1-equivalent}) as the winning condition of player~2. Note that the equivalence of \Cref{eq:energyDeterminacyPlayer2-1} and \Cref{eq:energyDeterminacyPlayer2-1-equivalent} still holds since $\varphi_c$ is still Borel for a fixed $c$. Therefore, these games are trivially determined. 

In this work, we will define the winning region of player~2 wrt \Cref{eq:energyDeterminacyPlayer2-2}, 
where $\varphi_c$
\begin{equation} \varphi_c = \energy_c^f = \begin{cases}\energy_c \cap \plays^f(G) &\text{ if } (G, E_f) \text{ is 1-fair} \\ 
  \energy_c \cup \plays(G) \setminus \plays^f(G) &\text{ if } (G, E_f) \text{ is 2-fair}\end{cases}
\end{equation}
That is, a fair energy game determined iff $\Win_1 \cup \Win_2 = Q$ where $\Win_1$ and $\Win_2$ are defined via \Cref{eq:energyDeterminacyPlayer1} and \Cref{eq:energyDeterminacyPlayer2-2}, respectively. 
We argue that the lack of equivalence between \Cref{eq:energyDeterminacyPlayer2-1} and \Cref{eq:energyDeterminacyPlayer2-2} prevents us from adapting a general gadget based approach for general fair energy games, as we do in fair mean-payoff games. This is because the translation 
of a fair energy game into a regular energy or mean-payoff game via gadgets, immediately implies determinacy (as in regular energy and mean-payoff games, two definitions of determinacy coincide). This points at the limits of the gadget based approach, and implies that they cannot be generalized smoothly to $\omega$-regular energy games. However, we show that 1-fair energy games are still determined in this sense, and we give a gadget-based solution algorithm for these games. 


==> sections/long-proof-of-1-fair-mp-gadget.tex <==
\begin{proof}[Proof of \cref{thm:mpgadgetcorrectness} for 1-fair mean-payoff games]
    We first show that $\Win_1(G') \, \cap \,Q \, \subseteq \,\Win_1(G)$ i.e., if player~1 wins the regular mean-payoff game from a node $q$ in $G'$, then player~1 also wins the fair mean-payoff game from $q$ in $G$ if $q$ is in $G$. 
    Let $\sigma'$ be a winning strategy for player~1 in $G'$ for the regular mean-payoff objective starting from node $q$ with $q \in \Win_1(G') \cap Q$. Without loss of generality, let $\sigma'$ be a positional strategy. We will construct a winning strategy $\sigma$ for player~1 in $G$ for the fair mean-payoff objective starting from node $q$.

   Consider the subgame arena $G'_{\sigma'}$ of $G'$ with respect to the strategy $\sigma'$. Note that all cycles in $G'_{\sigma'}$ are non-negative; else player~2 can force to eventually only visit a negative cycle and therefore construct a play in $G'_{\sigma'}$ with negative mean payoff value. This leads to a contradiction since $\sigma'$ is winning for player~1.

   Using $\sigma'$, we construct $\sigma$ in $G$ as follows:
   \begin{enumerate}[label=\alph*.]
       \item \label{item:1-fair-zeroth} If $q' \not \in Q^f$, then set $\sigma$ to be positional at $q'$ with $\sigma(q') = \sigma'(q')$. Note that this is well-defined since we do not use gadgets for nodes in $Q \setminus Q^f$.

       \item \label{item:1-fair-first} If $\sigma'(q') = q_r$ for some fair node $q' \in Q^f$, then set $\sigma$ to be positional at $q'$ with $\sigma(q') = \sigma'(q'_{\ESC})$. Intuitively this says if for a fair node $q'$, $\sigma'$ asks to choose the escape branch of the gadget, then $\sigma$ follows $\sigma'$ to choose that branch and moves to the corresponding `escape node' in $G$. 
       
       \item \label{item:1-fair-second} If $\sigma'(q') = q_l$ for some fair node $q' \in Q^f$, then we set $\sigma$ to be an infinite memory strategy at $q'$ that are played in rounds: consider an order on the fair successors of $q'$. In round $i \geq 0$, $\sigma$ chooses the `preferred sucessor'\RIT{what is prefered?} $\sigma'(q'_0)$ exactly $i$ times and then chooses the $i^\text{th}$ (modulo $|E_f(q')|$) fair successor. 
       
       % Formally, it keeps a counter $\counter$ for the rounds of the play, which is initialized at $1$; and a pointer $\mathbf{r}$ at the fair successors $E^f(p)$ of the node $p$. At round $\mathbf{i} = i$, $\sigma$ chooses the \enquote{preferred sucessor} $\sigma'(p_0)$ exactly $i$ times, and then takes the $\mathbf{r}^{th}$ fair successor once. Subsequently, it increments counter values of $\mathbf{i}$ and $\mathbf{r}$. When the value of $\mathbf{r}$ exceeds $|E^f(p)|$, it is reset to the first fair successor.
       % %local memory of size $\log(n^3W  +  n + |E^f(q)| + 2)$ make $s$ cycle through the set $\{s'(p_{0})\} \cup E^f(p)$ whenever it visits $p$, with a strategy that
       %spends substantially longer time at $p$s \enquote{preferred successor} $s'(p_{0})$ to collect enough positive weight, before it cycles
       %through its fair edges to fulfill the fairness condition. When $p$ is visited for the $k^{th}$ time, if $k \mod n^3W + n +2 \neq 0$, $s$ takes the edge $p \to s'(p_{0})$. 
       %If $k \mod n^3W  + n +2 = 0$, $s$ takes an edge in $E^f(p)$, starting from an arbitrary fair edge and cycling through all of them one-by-one whenever this condition holds.
   \end{enumerate}

   \noindent Now we prove that all $\sigma$ plays $\tau \in \plays_\sigma(G)$ are winning for player~1 in $G$. In particular, we will show that $\tau$ is fair and $\meanVal(\tau) \geq 0$.
   
   \smallskip
   For a play $\tau = q^0 q^1 \ldots \in \plays_\sigma(G)$, we construct its \emph{extension} $\tau'$ in $G'$ inductively as follows: we start with $q^0$ and $i=0$ and with increasing $i$,
   \begin{itemize}
     \item If $q^i \not \in Q^f$, append $\tau'$ with $q^{i+1}$;
     \item If $\sigma(H\cdot q^i)$ is defined using~\Cref{item:1-fair-first} i.e., $\sigma'(q^i) = q^i_r$ then append $\tau'$ with $\escape{q^i} \to q^{i+1}$. In particular, we append $\tau'$ with $q^i_r \cdot q^i_{\ESC}\cdot q^{i+1}$.
     \item If $\sigma(H \cdot q^i)$ is defined using~\Cref{item:1-fair-second}, then
       \begin{itemize}
         \item if $q^{i+1} = \sigma'(q^i_{0})$, append $\tau'$ with $\simul{q^i}\to q^{i+1}$ i.e., with $q^i_l \cdot q^i_{0} \cdot q^{i+1}$ ; 
         \item else, append $\tau'$ with $\fair{q^{i}} \to q^{i+1}$, i.e. $q^i_l \cdot q^i_\text{nW+1} \cdot q^{i+1}$.
       \end{itemize} 
   \end{itemize}

   Clearly, $\tau'$ is a play in $G'_{\sigma'}$ and hence it contains only non-negative cycles. Furthermore, the restriction of $\tau'$ to the nodes $Q$ of $G$, denoted by $\tau'|_Q$, is exactly $\tau$. 

   Let a `tail' of $\tau$ denote the infinite suffix $\tail$ of $\tau$ that contains only the nodes and edges visited infinitely often in $\tau$; and let $\tail'$ be the extension of $\tau$ in $G'$. We denote the subgraph of $G'_{\sigma'}$ restricted to the nodes and edges in $\tail'$ by $G'_{\tail'}$.

   We first show that $\tau$ is fair. Note that, it is sufficient to show that $\tail$ does not contain fair nodes $p$ for which $\sigma(p)$ is defined as~\Cref{item:1-fair-first}. This is because for all the fair nodes $p'$ in $\tail$, for which $\sigma(p')$ is defined as~\Cref{item:1-fair-second}, visits all their fair outgoing edges infinitely often in $\tau$ by the definition of $\sigma$. Let $p$ be a node for which $\sigma(p)$ is defined via~\Cref{item:1-fair-first}. Then $\sigma'(p) = p_r$. As $\sigma'$ is positional, among all the branches from the gadget of $p$, only $\escape{p}$ exists in $G'_{\sigma'}$ carrying the weight $-n^2W - n$. 
   Since from our assumption $p$ is visited infinitely often, there is a (simple) cycle in $G'_{\sigma'}$ that passes through $p$, and thus sees the weight $-n^2W -n$. This cycle must be non-negative
   since it is a cycle in $G'_{\sigma'}$, but in order to counteract the negative weight $-n^2W -n$, the cycle needs to contain $n$-many gadget edges with weight $nW+1$, which is not possible since there are at most $n-1$ many gadget edges with this priority in $G'_{\sigma'}$. With this argument, we conclude that $\tau$ is fair.
   
   Now we prove that $\meanVal(\tau) \geq 0$. First let us make an observation about the cycles in $G'_{\sigma'}$ that use only simulation branches. 

   \smallskip
   \begin{observation}[sim-cycles] We call cycles in $G'_{\sigma'}$ that do not contain any fair or escape branches \emph{sim-cycles}. That is, if there are any fair nodes on these cycles, only their simulation branches are in the cycle. Being part of $G'_{\sigma'}$, these cycles have non-negative weight.
   
   Since all the gadget edges on these cycles carry zero weight, when we restrict these cycles to non-gadget nodes $Q$, we get non-negative weight cycles in $G$ as well.
   That is, if $\mathbf{c'}$ is a simple sim-cycle in $G'_{\sigma'}$, then $\mathbf{c}|_{Q}$ is a non-negative cycle in $G$.
   \end{observation}
   
   We have shown above that $\tail$ contains no nodes for which $\sigma$ has been defined via~\Cref{item:1-fair-first}. Therefore, for all fair nodes $p$ in $\tail$, $\sigma$ is defined via~\Cref{item:1-fair-second}, and $G'_{\tail'}$ contains only the branches $\fair{p}$ and/or $\simul{p}$. Thus, all cycles in $\sigma'$ are either sim-cycles, or they visit a fair branch. 
   
   Now to show that $\meanVal(\tau) \geq 0$, we will use the following lemma which is easy to verify:
   
   \begin{remark}\label{lem:meanvalinfix}
     Given an infinite play $\rho$ and $\epsilon >0$, if there exists a natural number $k$ and a tail $\hat{\rho}$ of $\rho$ such that every $k$-length infix $\hat{\rho}_k$ of $\hat{\rho}$ satisfies $\meanVal(\hat{\rho}_k) \geq -\epsilon$, then $\meanVal(\rho) \geq -\epsilon$.
   \end{remark}
   Let $\epsilon > 0$ be arbitrary. Let $k\in \N$ such that $\frac{n^2W}{k} < \epsilon$. Since by our assumption $\tail$ has at least one fair node, \Cref{item:1-fair-second} is triggered infinitely often to construct the strategy $\sigma$. Therefore, the round (in the sense of~\Cref{item:1-fair-second}) will grow unboundedly bigger. Thus, we can get a tail $\tail$ of $\tau$ that is in round $k$. In $\tail$, for every fair node, their edge to their preferred successor is taken at least $k$-many times between any two occurrences of their other outgoing edges. Then in its extension $\tail'$ in $G'$, the simulation  branches of fair nodes are visited at least $k$-many times in between two occurences of fair branches.
   Therefore, in $\tail$ each infix $\tail_k$ of length $k$ visits the fair branch of each node at most once. Consequently, there are at most $n$-many simple cycles in $\tail_k$ that visits a fair branch, and all its other simple cycles are sim-cycles. Now, total weight of $n$-many simple cycles that are not sim-cycles are $\geq -n^2W$, and since all the sim-cycles have non-negative weight, $\meanVal(\tau_k) \geq \frac{-n^2W}{k} \geq - \epsilon$. Using the fact from the previous paragraph, we get that $\meanVal(\tau) \geq -\epsilon$. This implies that for any $\epsilon > 0$, $\meanVal(\tau) \geq -\epsilon$. Hence, $\meanVal(\tau) \geq 0$.

   This concludes the proof of the first direction. Now let us prove the other direction. In particular, we show that, if a node is winning for player~2 in $G'$, then it is also winning for player~2 in G i.e., $q \in \Win_2(G') \Rightarrow q \in \Win_2(G)$. 
 
   % We will fix an arbitrary node $v \in \sigma$ and show that in between each $2$ occurence of $v$s leftmost branch $\fair{v}$ in $\sigma'$, which corresponds to 
   % every time the edge $v \to v'$ is taken in $\sigma$ where $v'$ is not the preferred successor of $v$, the total energy is non-negative\ISin{??}. Furthermore, it will be clear from the argument that if for all nodes in $\sigma \cap Q^f$ their 
   % non-preferred successors are seen only finitely often in $\sigma$, then the total energy is monotonically increasing.

   % First let $\mathbf{u'} = \fair{v} \to u^0 \to u^1 \to \ldots u^k \to v$ be an infix of $\sigma'$ that starts and ends at $v$; where the branch following $\mathbf{u'}$ in $\sigma'$ is again $\fair{v}$, and
   % for no $u \in \sigma$ does $\fair{u}$ is seen in $\mathbf{u'}$ twice. 
   % In words, $\mathbf{u'}$ is an infix of $\sigma'$ inbetween two occurrences of the leftmost branch of $v$, and no other nodes 
   % take their leftmost branches twice in $\mathbf{u'}$.
   % Let $\mathbf{u} = \mathbf{u'}|_{Q}$, the image in $\mathbf{u'}$ in $G$. Clearly, $\mathbf{u}$ also starts and ends with $v$. We will show that $\energy(\mathbf{u}) \geq 0$\ISin{??}. 
   % Observe that at most $n$-many leftmost branches are seen in $\mathbf{u'}$. The rest of the branches are $0$-branches.
   % Also since $v$s leftmost branch is seen as the first edge and the following edge of $\mathbf{u'}$, 
   % the construction of $s$ implies that $v$ is seen $n^3W + n + 2$ times in $\mathbf{u'}$ (and in $\mathbf{u}$). So $\mathbf{u'}$ (and $\mathbf{u}$)
   % consists of $n^3W + n +1$-many cycles on $v$, whereas at most $n$ of these are non-$0$ cycles. 
   % The image of $n$-many non-$0$ cycles in $\mathbf{u'}$ can consist of at most $n^2$ nodes in $\mathbf{u}$ and therefore, can induce the least energy of $-n^2W$.
   % However since the rest of the cycles on $v$ are $0$-cycles and each contain at least one $0$-branch, $\simul{v}$; by our previous observation each has energy $n^3W + 1 - n^2W > (n-1)n^2W$.
   % Therefore, the total energy of $\mathbf{u}$ is non-negative. 

   % Now define $\mathbf{u'}$ and $\mathbf{u}$ as above, but let $\mathbf{u'}$ contain left branches $\fair{u}$ of nodes $u \neq v$ multiple times. That is, there can be at most $n-1$ that take their leftmost branches more than once in $\mathbf{u'}$.
   % We will show by induction that $\mathbf{u'}$ has positive energy.
   % \smallskip
   % \textit{Claim.} If there are $\leq n-k$-many nodes whose left branches are taken more than once in $\mathbf{u'}$ for some $k \in [1, n]$, then $\energy(\mathbf{u'}) > (k-1) n^2 W$.
   
   % \textit{Proof of claim.} For the base case, we take $k = n$, that is, no left branches repeat in $\mathbf{u'}$. This reduces to the case introduced in the previous paragraph, where we showed $\energy(\mathbf{u'}) > (n-1)n^2W$. 
   % As the inductive hypothesis, we assume the statement holds for $i \in [k+1, n]$, i.e. if $\mathbf{u'}$ has $\leq n-i$ nodes repeating their leftmost branches for some $i \in [k+1, n]$, then $\energy(\mathbf{u'}) > (i-1) n^2 W$. 
   % In the inductive step we show it for $k$, i.e. if $\mathbf{u'}$ has $\leq n-k$ nodes repeating their leftmost branches, $\energy(u') > (k-1) n^2 W$.
   % In a $\mathbf{u'}$ with $(n-k)$-many nodes repeating their leftmost branches, we can find infices $\mathbf{w^1}, \ldots, \mathbf{w^t}$ of $\mathbf{u'}$ for some $t \leq n-k$ such that each $\mathbf{w^i}$ starts with a leftmost branch of a node $w$ and ends with the same node, and the branch following $\mathbf{w^i}$ is again $\fair{w_i}$. 
   % Furthermore, $w_i \neq w_j$ for all $i \neq j \in [1, t]$. We can repeat this operation exhaustively such that if we remove the infices $\mathbf{w^1}, \ldots, \mathbf{w^t}$ from $\mathbf{u'}$, in the remaining sequence $\mathbf{u^{-}}:=\mathbf{u'} - (\mathbf{w^1}, \ldots, \mathbf{w^t})$, there are no repeating left branches. 

   
   % Note that the left branch of $w_i$ can be taken multiple times in $\mathbf{w^i}$.
   % If there is no leftmost branch repeating in $\mathbf{u'}$, then we obtain the desired inequality from the base case. 
   % Otherwise, we can always find at least such infix, $\mathbf{w^1}$.
   % If in a $\mathbf{w^i}$, the left branch of $w_i$ repeats, then we can view $\mathbf{w^i}$ as a concetanation $\mathbf{w^i}_1\cdot \mathbf{w^i}_2 \cdots \mathbf{w^i}_p$ such that each $\mathbf{w^i}_j$ for $j \in [1, p]$ starts with $\fair{w_i}$, ends with $w_i$, and $\fair{w_i}$ is not repeated.
   % If the left branch of $w_i$ does not repeat in $\mathbf{w^i}$, then simply, $\mathbf{w^i} = \mathbf{w^i}_1$.
   % Note that in each $\mathbf{w^i}_j$, there are at most $(n-k-1)$-nodes repeating their leftmost branches. 
   % Then, by the inductive hypothesis, $\energy(\mathbf{w^i}_j) > (k+1) n^2 W$, and therefore  $\energy(\mathbf{w^i}) > p \cdot (k+1) n^2 W \geq (k+1) n^2 W $ for every $\mathbf{w^i}$.

   % Recall that in $\mathbf{u^{-}}$ there are no repeating left branches. That is, there are at most $n$-many left branches. By an argument similar to before, we know that there can be at most $n$-many simple non-$\varepsilon$ cycles, and they can cause 
   % at the worst, $-n^2W$ negative energy. This is because $\epsilon$-cycles have positive energy.
   % Since we assumed $\mathbf{u^{-}}$ has at least one infix $\mathbf{w^1}$ with energy larger than $(k+1) n^2 W$; we get that $\energy(\mathbf{u'}) > (k+1) n^2 W - n^2 W = k n^2 W$.
   % This finishes the proof of the claim. \qed

   % If there are no nodes in $\sigma$ that take their left branch in $\sigma'$, then all cycles in $\sigma'$ are $\varepsilon$-cycles, and therefore every cycle in $\sigma$ have non-negative\ISin{positive} energy. 

   % As $\sigma'$ can be seen as an infinite concetanation of infices $\mathbf{u'}$ of bounded size (due to the finiteness of $G'$), we can conclude that $\energy(\sigma)\geq 0$\ISin{$\energy(\sigma_i)$ goes to infinity in the limit} in both cases, which finalizes the proof of $(\Rightarrow)$.\ISinside{Not quite. We need a bit more. Explained above.} Now we prove the second direction.

   \smallskip
    Analogous to the previous part, we consider a positional winning strategy $\pi'$ of player~2 in $G'$ and construct, this time, a \emph{positional} winning strategy $\pi$ for player~2 in $G$. Note that, none of the fair nodes in $G$ belong to player~2 and hence the construction of $\pi$ is quite straight forward: for all $q \in Q_2$, we set $\pi(q) = \pi'(q)$. We define $G'_{\pi'}$ as the subgame restricted to the strategy $\pi'$, as before. 

   For a play $\tau = q^0 q^1 \ldots \in \plays_\pi(G)$, we define its \emph{extension} $\tau'$ in $G'$ inductively as follows: we start from with $q^0$ and $i = 0$, and with increasing $i$,
   \begin{itemize}
       \item If $q^i \not \in Q^f$, append $\tau'$ with $q^{i+1}$; Otherwise,
       \item If $\simul{q^i}$ exists in $G'_{\pi'}$, append $\tau'$ with $q^i_l \cdot q^i_{0} \cdot q^{i+1}$;
       \item If $\simul{q^i}$ does not exist in $G'_{\pi'}$:
       \begin{itemize} 
           \item If $q^{i+1} = \pi'(q^i_\text{nW+1})$, append $\tau'$ with the fair branch i.e. $q^i_l \cdot q^i_\text{nW+1} \cdot q^{i+1}$, 
           \item Otherwise, append it with the escape branch, i.e. $q^i_r \cdot q^i_{\ESC} \cdot q^{i+1}$.
       \end{itemize}
   \end{itemize}
  % We define $\sigma$, $\sigma'$ and $G'_{\sigma'}$ as before. 
   We define the tail of $\tau$ as $\tail$ and its extension $\tail'$, analogous to the previous part. We denote the subgraph of $G'_{\pi'}$ restricted to the nodes and edges in $\tail'$ by $G'_{\tail'}$.

   Let $\tau \in \plays_\pi(G)$ be a play in $G$ that conforms with $\pi$. If $\tau$ is not fair, it is automatically won by player~2. Therefore, let us assume that $\tau$ is fair. We will show that all the simple cycles in $\tail$ has negative weight. To prove this, we will use the fact that its extension $\tau'$ is a play in $G'_{\pi'}$ and hence all the cycles in $G'_{\tail'}$ have negative weight as $\pi'$ is winning for player~2 for the mean-payoff objective in $G'$. Since the length of simple cycles are bounded by $n$, this gives us $\meanVal(\tau) < 0$.

   Our main argument is the absence of fair branches in $G'_{\tail'}$, which we introduce in \emph{Claim 1}. 
   
   \smallskip 
   \begin{claim}\label{claim:1-fair-absence}
     If $\tau$ is fair, there exist no fair branches $(\fair{})$ in $G'_{\tail'}$.
   \end{claim}

   \noindent Before proving the claim, we first discuss how~\Cref{claim:1-fair-absence} implies that all simple cycles in $\tail$ are negative, resulting $\meanVal(\tau) < 0$. From the definition of extension, absence of fair branches in $G'_{\tail'}$ implies that either (i) for all $q \in Q^f$ only $\simul{q}$ exists in $G'_{\tail'}$, or (ii) for some $q \in Q^f$, only the escape branch $\escape{q}$ exists in $\tail'$. By construction of $\tau'$, case (ii) above implies that there exists a fair node $q \in Q_f$ that appears infinitely often in $\tau$ but does not take all its fair outgoing edges, in particular $q \to \pi'(q_\text{nW+1}) \in E^f(q)$ infinitely often. This implies that $\tau$ is unfair, contradicting our assumption. In case of (i), since all simple cycles $\mathbf{c}'$ in $\tail'$ are negative and none of the gadget nodes contribute any weight due to only simulation branches being seen, we conclude that the corresponding cycles $\mathbf{c} = \mathbf{c'}|_{Q}$ in $\tail$ have negative weight. This implies that $\meanVal(\tau) < 0$. 
   
   By the above mentioned argument, proving~\Cref{claim:1-fair-absence} is sufficient to prove the overall direction. We now prove the claim.
    
    \smallskip
   \noindent \textit{Proof of~\Cref{claim:1-fair-absence}.} As we have discussed above, since $\tau$ is fair, whenever $\escape{q}$ is in $G'_{\tail'}$ for a node $q \in Q^f$, $\fair{q}$ is also in $G'_{\tail'}$.
   Now let us remove all the escape branches $\escape{q}$ of all nodes $q \in Q^f$ from $G'_{\tail'}$ and construct a subgraph $S$. Note that $S$ has no dead-ends, since for all $q$ for which $\escape{q}$ got removed from $G'_{\tail'}$, $\fair{q}$ was also in $G'_{\tau'}$, and hence it is in $S$.
   
   Now, for all nodes $q$ in $S$, either its fair branch or its simulation branch is in $S$. Note that since it is a subgraph of $G'_{\pi'}$, all cycles in $S$ have negative weight. It is easy to see that a node $q\in Q^f$ for which $\fair{q}$ is in $S$, cannot lie on a cycle in $S$. This is true because a fair branch carries weight $nW+1$. The other edges in a simple cycle in $S$ are either gadget edges carrying weight $0$ (note that, we have assumed that the fair branches are not present in $S$) or edges in $G$ carrying weight $\geq -W$. Hence, any simple cycle containing a fair branch would have positive weight contradicting that S has all simple cycles with negative weight.
   
   Now assume fair branches exist in $\tail'$, but not on cycles in $S$. Then all cycles in $S$ consist only of simulation branches. However, nodes with simulation branches have the same outgoing edges in 
   $G'_{\tail'}$ as in $S$. Recall that every node in $S$ is visited infinitely often in $\tau$. Since $S$ has no dead-ends, it contains a cycle. Then $\tau$ will eventually visit a node on a cycle of $S$. Since this node will have the same outgoing edges in $S$ and $\tail'$, $\tau$ will never leave the cycles of $S$, which only have simulation branches. 
   This implies that fair branches are not visited after some point on in $\tau$, and contradicts our assumption that fair branches exist in $\tail'$.
   \qed
   With this, we conclude the proof of the second direction, and that of the theorem.
\end{proof}

==> sections/mean-payoff.tex <==
In this section, we explore the connections between fair energy games and fair mean-payoff games.
While finite memory is enough for winning strategies in fair energy games, we show that the optimal strategies in fair mean-payoff games may require infinite memory. 
Despite this difference, we show that there is a tight relationship between the two. 
Specifically, we show that fair energy games are polynomially equivalent to fair mean-payoff games, leading to an algorithm for solving fair mean-payoff games with a similar complexity to that of fair energy games.

It is well-known that there is a strong connection between energy games and mean-payoff games. However, given that finite memory is enough for winning strategies in fair energy games, it is not the case for optimal strategies in fair mean-payoff games. To see this, consider the following example.
    

As shown in the example above, one can use the idea of an infinite memory strategy playing in rounds to show that the optimal values in a fair mean-payoff game is same as the optimal value in a mean-payoff game restricted to a subset of nodes. 
\begin{lemma}\label{lemma:mean-payoff}
    Let $v$ be the optimal value and $\sigma$ be an optimal strategy of player~$1$ from node $q_0$ in fair mean-payoff game $(G = (Q,E,w),E_f,\meanpayoff)$. Let $Q' = \bigcup_{\tau\in\plays_\sigma(G,q_0)}\inf(\tau)$ be the set of nodes visited infinitely often by $\sigma$-plays from~$q_0$. Suppose $q_0 \in Q'$.
Then, $v$ is also the optimal value from node $q_0$ in mean-payoff game $(G' = (Q',E',w),\meanpayoff)$ with $Q_i' = Q_i\cap Q'$, and $E' = E \cap (Q' \times Q')$.
\end{lemma} 
\begin{proof}
Let $v'$ be the optimal value and $\sigma'$ be an optimal positional strategy of player~$1$ from node $q_0$ in mean-payoff game $(G',\meanpayoff)$. 
We want to show that $v = v'$.
As $\sigma$ is a winning strategy in fair mean-payoff game $(G,E_f,\meanpayoff(v))$ from $q_0$, it holds that $\plays_\sigma(G,q_0)\subseteq \meanpayoff(v)$.
Hence, $\sigma$ is also a winning strategy for player~$1$ from $q_0$ in mean-payoff game $(G,\meanpayoff(v))$. As $v'$ is the optimal value for this game, it holds that $v'\geq v$.
We only need to show that $v\geq v'$.

First, note that every $\sigma$-play from $q_0$ in $G$ is fair. Hence, for every fair edge $(q,q')$ with $q \in Q'$, if a play in $\plays_\sigma(G,q_0)$ visits $q$ infinitely often, then it also uses the fair edge $(q,q')$ infinitely often, which implies $q' \in Q'$. 
Therefore, every fair play in $(G',E_f')$ from $q_0$ with $E_f' = E_f \cap (Q' \times Q')$ is also a fair play in $(G,E_f)$.
Furthermore, as every $\sigma$-play from $q_0$ eventually stays in $Q'$, there is no edge of player~$2$ from $Q'$ to $Q\setminus Q'$ in $G$, i.e., $E \cap (Q_2' \times (Q\setminus Q')) = \emptyset$. 

Now, consider the strategy $\sigma''$ for player~$1$ in $G$ that is played in rounds for every node $q\in Q'$ as follows: in round $i\geq 0$, the strategy plays $q\rightarrow \sigma'(q)$ for first $i$ times $q$ is visited in the play, then it plays each fair edge in $qE_f'$ once for the next $\abs{qE_f'}$ times $q$ is visited in the play, and progresses to round $i + 1$. 

To prove $v\geq v'$, as $v$ is the optimal value from $q_0$ in $(G,E_f,\meanpayoff)$, it is enough to show that $\sigma''$ is a winning strategy for player~$1$ in fair mean-payoff game $(G,E_f,\meanpayoff(v'))$ from $q_0$.
Let $\tau$ be a $\sigma''$-play from $q_0$ in $G$. 
As player~$2$ doesn't have an edge from $Q'$ to outside, $\tau$ is also a play in $G'$.
Due to the second phase of $\sigma''$, it is easy to see that $\tau$ is fair in $(G',E_f')$, and hence, it is fair in $(G,E_f)$.
It remains to show that the mean-payoff value of $\tau$ is at least $v'$.

Consider the suffix $\tau'$ of $\tau$ where the strategy $\sigma''$ already has played $k > 2W\abs{Q}^2$ rounds for each node in $\inf(\tau)$.
Consider an infix $\tau''$ of $\tau'$ of length~$k$. 
By construction of $\sigma''$, a fair edge cannot be used twice in $\tau''$.
So, $\tau''$ consists of at most $\abs{E_f'}$ fair edges, and at every other node, $\sigma''$ plays according to $\sigma'$. 
Hence, in these segments where $\sigma''$ plays according to $\sigma'$, except for small parts (of size less than $|Q'|$) before and after the fair edges, all others consist of cycles of $G_{\sigma'}$, which have by definition, an average weight of at least~$v'$. 
Therefore, the average weight of $\tau''$ is at least 
\[\frac{(k-2\abs{Q'}\abs{E_f'})\cdot v' - 2\abs{Q'}\abs{E_f'}\cdot W}{k}
= v' - \frac{2\abs{Q'}\abs{E_f'} (v'+W)}{k}.\]  
As there are infinitely many rounds for every node in $\inf(\tau)$, the limit of the average weight of $\tau$ is at least
\[\lim_{k\rightarrow \infty} \left(v' - \frac{2\abs{Q'}\abs{E_f'} (v'+W)}{k}\right) = v'.\]
Hence, $\sigma''$ is a winning strategy for player~$1$ in fair mean-payoff game $(G,E_f,\meanpayoff(v'))$ from $q_0$.\qed
\end{proof}

Due to the above lemma, the rationality of optimal values in mean-payoff games is also retained in case of fair mean-payoff games.
\begin{lemma}\label{lemma:mean-payoff-rational}
    Given a fair mean-payoff game $(G,E_f,\meanpayoff)$ with set $Q$ of nodes and weight function $w:E\rightarrow [-W,W]$, the optimal value from any node is a rational number in $\mathbb{Q}_G$, where $\mathbb{Q}_G = \{\frac{a}{b} \mid 1\leq a\leq \abs{Q}, \abs{b}\leq a\cdot W\}$.
\end{lemma}
\begin{proof}
    Let $v$ be the optimal value and $\sigma$ be an optimal strategy of player~$1$ from node $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff)$. Let $Q' = \bigcup_{\tau\in\plays_\sigma(G,q_0)}\inf(\tau)$ as in \Cref{lemma:mean-payoff}.
As every $\sigma$-play from $q_0$ eventually enters $Q'$, it is easy to see that $v$ is also the optimal value from one of the nodes $q_0'\in Q'$. 
By \Cref{lemma:mean-payoff}, $v$ is also the optimal value from $q_0'$ in the mean-payoff game restricted to $Q'$. As the optimal value in any mean-payoff game with $(G,\meanpayoff)$ belongs to $\mathbb{Q}_G$~\cite{}, it holds that $v\in\mathbb{Q}_G$.
\qed
\end{proof}

As we saw earlier, the optimal strategy may require infinite memory in fair mean-payoff games. However, we next show that, for suboptimal values, finite memory is enough for a winning strategy of player~1.
\begin{lemma}\label{lemma:mean-payoff-finite}
    Given a fair mean-payoff game $(G,E_f,\meanpayoff)$, let the optimal value from some node $q_0$ is $v$. Then, for all $\epsilon > 0$, there exists a finite-memory strategy of player~$1$ that is winning from $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff(v-\epsilon))$.
\end{lemma}
\begin{proof}
    Let $v$ be the optimal value and $\sigma$ be an optimal strategy of player~$1$ from node $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff)$. Let $Q' = \bigcup_{\tau\in\plays_\sigma(G,q_0)}\inf(\tau)$, $E' = E \cap (Q' \times Q')$, and $E_f' = E_f \cap (Q' \times Q')$ as in \Cref{lemma:mean-payoff}.

Suppose $q_0 \in Q'$.
By \Cref{lemma:mean-payoff}, player~$1$ can win from $q_0$ in mean-payoff game $(G',E_f',\meanpayoff(v))$ with $G' = (Q',E',w)$.
Let $\sigma'$ be a memoryless strategy for player~$1$ that is winning from $q_0$ in $(G',E_f',\meanpayoff(v))$.
Let $k\in\N$ such that 
\[\frac{2\abs{Q'}\abs{E_f'} (v'+W)}{k} < \epsilon.\]
Now, consider the strategy $\sigma'$ for player~$1$ in $G$ that is played in rounds for every node $q\in Q'$ as follows: in each round, the strategy plays $q\rightarrow \sigma(q)$ for first $k$ times $q$ is visited in the play, then plays each fair edges in $qE_f'$ once for the next $\abs{qE_f'}$ times $q$ is visited in the play, and progresses to next round. Note that, the strategy plays the same way in every round, and hence, it has finite-memory. 

As in the proof of \Cref{lemma:mean-payoff}, it is easy to see that every $\sigma'$-play $\tau$ from $q_0$ is fair and all of its infix of length $k$ has an average weight of at least $v- \frac{2\abs{Q'}\abs{E_f'} (v'+W)}{k} > v-\epsilon$. Hence, the mean-payoff value of $\tau$ is at least $v-\epsilon$.
Therefore, $\sigma'$ is a finite-memory winning strategy for player~$1$ in fair mean-payoff game $(G,E_f,\meanpayoff(v-\epsilon))$ from $q_0$.

Now, suppose $q_0 \notin Q'$. As every $\sigma$-play from $q_0$ eventually stays in $Q'$, there is a finite-memory strategy $\sigma''$ for player~$1$ that ensures that every $\sigma''$-play from $q_0$ eventually stays in $Q'$. One can obtain a strategy for player~$1$ that follows $\sigma''$ until it reaches some node $q_0'$ in $Q'$ and then follows $\sigma'$ (constructed for $q_0'$) for the rest of the play. This strategy is a finite-memory strategy that is winning from $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff(v-\epsilon))$. 
\qed
\end{proof}




With the above essential properties, we are ready to present the equivalence between fair energy games and fair mean-payoff games.
\begin{theorem}\label{thm:mean-payoff-equivalence}
    Let $(G,E_f)$ be a fair game arena with $G = (Q,E,w)$, and let $\epsilon = \frac{1}{\abs{Q}+1}$ and $v\in\mathbb{Q}_G$ be rational numbers. Then, player~$1$ has a winning strategy from $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff(v))$ if and only if player~$1$ has a winning strategy in fair energy game $(G',E_f,\energy)$ with $G' = (Q,E,w')$ such that $w'(q) = w(q) -v+\epsilon$ for all $q\in Q$.
\end{theorem}
\begin{proof}
Let us prove both directions of the equivalence.
\paragraph*{\textbf{$(\Rightarrow)$}} Let player~$1$ has a winning strategy from $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff(v))$. 
By \Cref{lemma:mean-payoff-finite}, there exists a finite-memory strategy $\sigma$ for player~$1$ that is winning from $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff(v-\epsilon))$.
Now, consider a cycle $C$ reachable from $q_0$ in $G_\sigma$.
By definition, there is a $\sigma$-play $\tau_C$ in $G$ that eventually loops in $C$ and still has an average weight of at least $v-\epsilon$. Hence, the average weight of the cycle $C$ in $G$ is at least $v-\epsilon$. Therefore, the average weight of the cycle $C$ in $G'$ is at least $0$.
Furthermore, by definition of $\sigma$, play $\tau_C$ is also fair, and hence, $C$ uses every enabled fair edges.
So, every cycle reachable from $q_0$ in $G'_\sigma$ is non-negative and uses every enabled fair edges. 
As every $\sigma$-play $\tau$ from $q_0$ eventually (i.e., after fewer than $\abs{Q}$ steps) only uses the cycles in $G'_\sigma$, it must hold that $\tau$ is fair and the weight $\abs{Q}W+ w(\tau,i) \geq 0$ for all $i\in\N$.
Hence, $\sigma$ is a winning strategy for player~$1$ in fair energy game $(G',E_f,\energy(\abs{Q}W))$.

\paragraph*{\textbf{$(\Leftarrow)$}} Conversely, let player~$1$ has a (finite-memory) winning strategy $\sigma$ from $q_0$ in fair energy game $(G',E_f,\energy)$.
Consider a cycle $C$ reachable from $q_0$ in $G'_\sigma$.
By construction, there is a $\sigma$-play $\tau_C$ in $G'$ that eventually loops in $C$ and has a non-negative total weight. Hence, the average weight of the cycle $C$ in $G'$ is at least $0$. Therefore, the average weight of the cycle $C$ in $G$ is at least $v-\epsilon$.
Furthermore, by definition of $\sigma$, play $\tau_C$ is also fair, and hence, $C$ uses every enabled fair edges.
So, every cycle reachable from $q_0$ in $G_\sigma$ is fair and has average weight at least $v-\epsilon$ in $G$.
As every $\sigma$-play $\tau$ from $q_0$ eventually only uses the cycles in $G_\sigma$, it must hold that $\tau$ is fair and the average weight $\tau$ is at least $v-\epsilon$ in $G$.
Hence, $\sigma$ is a winning strategy for player~$1$ in fair mean-payoff game $(G,E_f,\meanpayoff(v-\epsilon))$.
Therefore, the optimal mean-payoff value in $(G,E_f)$ is at least $v-\epsilon$.

By \Cref{lemma:mean-payoff-rational}, the optimal mean-payoff value in $(G,E_f)$ is a rational number in $\mathbb{Q}_G$. 
As $v\in \mathbb{Q}_G$ and $\epsilon = \frac{1}{\abs{Q}+1}$, the smallest rational number in $\mathbb{Q}_G$ that is at least $v-\epsilon$ is~$v$.
Therefore, the optimal mean-payoff value in $(G,E_f)$ is at least~$v$, and hence, player~$1$ has a winning strategy from $q_0$ in fair mean-payoff game $(G,E_f,\meanpayoff(v))$.\qed
\end{proof}










